Improving the Fidelity of CNOT Circuits on NISQ Hardware

We introduce an improved CNOT synthesis algorithm that considers nearest-neighbour interactions and CNOT gate error rates in noisy intermediate-scale quantum (NISQ) hardware. Compared to IBM's Qiskit compiler, it improves the fidelity of a synthesized CNOT circuit by about 2 times on average (up to 9 times). It lowers the synthesized CNOT count by a factor of 13 on average (up to a factor of 162). Our contribution is twofold. First, we define a $\textsf{Cost}$ function by approximating the average gate fidelity $F_{avg}$. According to the simulation results, $\textsf{Cost}$ fits the error probability of a noisy CNOT circuit, $\textsf{Prob} = 1 - F_{avg}$, much tighter than the commonly used cost functions. On IBM's fake Nairobi backend, it matches $\textsf{Prob}$ to within $10^{-3}$. On other backends, it fits $\textsf{Prob}$ to within $10^{-1}$. $\textsf{Cost}$ accurately quantifies the dynamic error characteristics and shows remarkable scalability. Second, we propose a noise-aware CNOT routing algorithm, NAPermRowCol, by adapting the leading Steiner-tree-based connectivity-aware CNOT synthesis algorithms. A weighted edge is used to encode a CNOT gate error rate and $\textsf{Cost}$-instructed heuristics are applied to each reduction step. NAPermRowCol does not use ancillary qubits and is not restricted to certain initial qubit maps. Compared with algorithms that are noise-agnostic, it improves the fidelity of a synthesized CNOT circuit across varied NISQ hardware. Depending on the benchmark circuit and the IBM backend selected, it lowers the synthesized CNOT count up to $56.95\%$ compared to ROWCOL and up to $21.62\%$ compared to PermRowCol. It reduces the synthesis $\textsf{Cost}$ up to $25.71\%$ compared to ROWCOL and up to $9.12\%$ compared to PermRowCol. Our method can be extended to route a more general quantum circuit, giving a powerful new tool for compiling on NISQ devices.

==> scripts/6-disc.tex <==
\section{Open Research Problems and Discussions}
\label{sec:open problems}
%\subsection{Where do the improvements come from?}
%\subsection{Find an Approximation Form of Fidelity with an Arbitrary Circuit}
\subsection{Improve the Accuracy of our Cost Function}
\sarah{In this paper, we only concern the CNOT gate error rate and ignore the errors on the idling qubits. Therefore, every CNOT circuit can be simplified as a consecutive noisy channel. The error probability of its horizontal component is given by each noisy CNOT gate. The major room for improvement is to account for the errors resulting from the T1/T2 time. Once we know how to characterize the errors on idling qubits, we can generalize our cost function to work with a noisy single-qubit gate. 

In \cref{subsec:parallel error channel}, we provide two approximated forms of the average gate fidelity of a parallel error channel. We are not sure which cost function provides a more accurate measure for the quality of $\mathbf{C}$. In addition, we cannot yet determine how the cost functions of a parallel and consecutive error channels interact with each other. We conjecture that it might be more accurate to model a noisy quantum circuit as a mix of parallel and consecutive error channels. 
 }
Within this paper, our examination has been confined to CNOT error rates, with the assumption that no additional errors such as decoherence or crosstalk are present. Guided by this assumption, we derived an approximate representation for the average gate fidelity specific to CNOT circuits. However, in our endeavor to broaden the scope of our method for the resynthesis of diverse circuits, a need arises to contemplate a fresh approximate form. This revised form should account for other errors, especially those linked to single-qubit gates.
\subsection{Apply our error mitigation techniques to routing an arbitrary quantum circuit}
Ultimately, our goal is to adapt the \textit{NAPermRowCol} so that it routes an arbitrary quantum circuit rather than just the CNOT circuits in a NISQ hardware. To this end, we consider the ``Slice-and-Build'' method~\cite{gheorghiu2022reducing} and the ``CNOT-Comb synthesis'' method~\cite{murphy2023global}. Suppose that we are given a circuit over the Hadamard gates, the phase gates, the CNOT gates, and the T gates, alongside an IBM fake backend. These two methods are detailed below.
\vspace{-1em}
\subsubsection{The Slice-and-Build Method}
Starting from the lefthand side of the circuit, we partition it into subcircuits based on the locality of the Hadamard gates. This means the circuit is sliced into subcircuits, each of which is composed of only the phase gates, CNOT gates, and T gates. Then route each subcircuit independently while considering the NN interactions and the gate error rates. Since each subcircuit consists of only the CNOT gates and $R_Z$ rotations, we could use the phase polynomial network \cite{amy2014polynomial} to represent the semantics of each subcircuit. Next, we adapt our error mitigation strategies by considering the single-qubit gate error rate, the relaxation error, and the decoherence. After routing each subcircuit, piece them back together according to the locality of the Hadamard gates.

%The approach is dividing an arbitrary circuit into subcircuits, synthesizing each subcircuit separately, and then merging them. When dealing with circuits containing CNOT and Rz rotations, the use of phase polynomials facilitates representation. Thus, by segmenting the circuit at the H gate location and synthesizing individual segments concurrently, we can later integrate these resynthesized subcircuits to achieve the resynthesis of the entire circuit. 

\subsubsection{The "CNOT-Comb" resynthesis} 
    In the CNOT-Comb resynthesis approach, temporal qubits are important in synthesizing CNOT circuits alongside single-qubit gates. Within this methodology, we allocate the temporal qubits to correspond with the positions of single-qubit gates in the circuit. The fundamental notion of the extractibility of the ith qubit is pivotal, signifying the thorough resynthesis of the parity term linked to the ith qubit. With n representing the total count of logical qubits and m denotes the total number of additional temporal qubits, the submatrix utilized for parity resynthesis consistently maintains dimensions of n(n+m). Through subsequent resynthesis utilizing this submatrix, we attain a circuit with the same semantic meaning as the original circuit.
\vspace{2em}
\subsection{Improve the Algorithm NAPermRowCol}
The necessity to integrate ancilla qubits in the routing process has become apparent. Qiskit's routing approach utilizes ancilla qubits to establish connections between non-adjacent qubits. If qubit 2, for instance, is designated as an ancilla qubit, CNOT operations involving its neighbors facilitate the connection of other qubits. However, our algorithm, along with others like ROWCOL, is different from this approach by not employing ancilla qubits and treating them as isolated entities. Essentially, ancilla qubits are removed from the graph, leading to suboptimal routing outcomes. This is due to the necessity of detours for CNOT operations, given the inability to traverse ancilla qubits. We are currently exploring the expansion of our routing methods to incorporate ancilla qubits and plan to compare the results.    

\subsection{Find the Lower Bound of the Synthesis Result}
We have substantiated the superiority of our approach over alternative methods through a comparative analysis of costs. Our evaluation involved generating results for 100 ciruits across varying quantities of qubits and distinct original CNOT counts. The reduction in errors in the benchmarking results sufficiently supports our claim regarding the efficacy of our method. However, considerations about sub-optimality necessitate a deeper examination. Specifically, how closely does our outcome align with the optimal value? To address this question, we intend to compute the lower bound based on factors such as the original circuit, topology, and the error distribution of CNOTs. The lower bound serves as a benchmark, representing the optimal result attainable, beyond which further reduction in the cost of the resynthesized circuit becomes unattainable.


%\item Use ZX diagram to optimize the NISQ problem




==> scripts/7-conclu.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this work, we propose an improved noise-aware CNOT routing algorithm that exploits empirical data on NISQ hardware. Firstly, we define a cost function $\Cost$ to gauge the quality of a noisy CNOT circuit. This is done by approximating the average gate fidelity $F_{avg}$. Based on the simulation results on IBM's fake Nairobi backend, $\Cost$ fits the error probability of a noisy CNOT circuit, $\Prob = 1 - F_{avg}$, with the maximum approximation error lower than $10^{-3}$. On other backends, $\Cost$ fits $\Prob$ consistently better than the other cost functions. Moreover, it circumvents the computation complexity of calculating $F_{avg}$ and shows remarkable scalability.

%error mitigation strategy for synthesizing a CNOT circuit on noisy intermediate-scale quantum (NISQ) hardware. Our case study is carried out on IBM's superconducting quantum computers and we account for two physical constraints: the nearest-neighbour interactions and the CNOT gate error rates. As a first attempt, we assume no parallelization of CNOT gates and no noise on idle qubits. Additionally, we use a generalized Pauli channel to model noises. 



Next, we use $\Cost$ to design an architecture-aware CNOT synthesis algorithm, NAPermRowCol. It is inspired by the algorithm GENNS and built upon the algorithm PermRowCol. It reduces a CNOT synthesis algorithm to a Steiner tree problem and lowers the CNOT count by factoring out SWAP gates after the synthesis. Moreover, it uses noise-aware heuristics to make an informed decision at each reduction step. NAPermRowCol is benchmarked against the state-of-the-art CNOT synthesis algorithms according to the $\Cost$ metric and the synthesized CNOT count. It performs significantly better than the Qiskit transpiler, especially for circuits with a larger CNOT count. Compared with algorithms that are noise-agnostic, it lowers the synthesized CNOT count and is much cheaper for routing random CNOT circuits of different sizes. %For example, to route a 7-qubit CNOT circuit, it is about $30\%$ cheaper than ROWCOL and $10\%$ cheaper than PermRowCol on all of the benchmarked backends. 
Overall, NAPermRowCol is effective and scalable in reducing the CNOT count and minimizing the error probability of a synthesized CNOT circuit. 

Our paper paves the way for numerous compelling research questions, each of which invites further exploration. As a first attempt, we assume no parallelization of CNOT gates and no noise on idle qubits. Additionally, we use a generalized Pauli channel to model noise. These assumptions make our cost functions less general. A major room for improvement is to account for the errors resulting from the T1/T2 time and noisy single-qubit gates. This will help us design an improved architecture-aware synthesis algorithm for quantum circuits over a universal gate set. Second, while generalized Pauli channels are a useful and widely applicable model in quantum information, they do not encompass all possible completely positive maps (e.g., more complex multi-qubit interactions, non-Pauli types of noise and decoherence). Modelling a noisy quantum circuit with a more general channel representation is an important avenue for future work. Finally, NAPermRowCol shows modest improvements when synthesizing a CNOT circuit over more than 16 qubits. Investigation of its performance as quantum systems scale in terms of qubit width and circuit complexity is an open problem. 
% Can we investigate its performance as quantum systems scale in terms of qubit count and circuit complexity? What are the computational overheads with respect to the hardware specifics, and how can these be minimized?


%In this paper, we propose a physical constraint-aware routing algorithm called \textit{NAPermRowCol} and demonstrate its advantage in improving the fidelity of CNOT circuits on NISQ hardware. It is built on the algorithm \textit{PermRowCol}~\cite{griendli2022}, which is aware of the underlying hardware architecture but is not sensitive to the noises in the system. The benchmark results, conducted on IBM’s FakeCairo, FakeMelbourne, and FakeNairobi backends, clearly show the improvement of \textit{NAPermRowCol} over the state-of-the-art algorithms such as \textit{RowCol}, \textit{PermRowCol}, and the standard Qiskit transpiler algorithm.

%The key metrics of comparison included CNOT counts, accumulated CNOT gate error rates, and error probabilities. \textit{NAPermRowCol} consistently showed lower CNOT counts and error rates across various qubit subregions, ranging from 5 to 20 qubits. These benchmark results indicate that \textit{NAPermRowCol} is not only effective in reducing the CNOT counts, which is a primary source of errors in quantum circuits, but also in minimizing the overall error probabilities. Therefore, \textit{NAPermRowCol} enhances the reliability of quantum computations on NISQ devices.

%One notable aspect of our research is the focus on realistic quantum computing environments, where noise and error are inevitable. By optimizing for these factors, \textit{NAPermRowCol} represents a significant step towards practical quantum computing, providing a more robust and efficient approach to quantum circuit synthesis and routing in the presence of hardware constraints and errors.

%In conclusion, \textit{NAPermRowCol} emerges as a powerful tool for optimizing CNOT circuits, particularly in the context of NISQ technologies. Further afield, we plan to extend these techniques to a large class of quantum circuits (e.g., the Clifford$+$T circuits) and incorporate other types of errors beyond just the CNOT gate errors. This would further solidify the algorithm's applicability and utility in real-world quantum computing scenarios.


==> scripts/8-1-intuitionBehindPermRowCol.tex <==
\section{Intuition Behind the PermRowCol}
\label{sec: intuition PermRowCol}

==> scripts/8-1-subroutines.tex <==
\section{Subroutines}

% ChooseVertex
\Minyoung{I have to check this}
\begin{algorithm}[H]
   \begin{algorithmic}[1]
       \State \textbf{input } The connectivity graph $G = (V_G, E_G, \omega_G)$ and the parity matrix \vect{A}.
       \State \textbf{output} The vertex $v$ that has the minimum Hemming weight and the minimum metric
       \State $M \gets \{\}$;
       \State $\Candidates \gets $\textbf{NonCuttingVertex}$(V_G, E_G)$;
        \For {$v$ in $\Candidates$};
        \For {$u$ in $v$.neighbours};
        \State $e \gets E_G[(u,v)]/|v.\text{neighbours}|$
        \EndFor
        \State $M[v] \gets $\textbf{HammingWeight}$(\vect{A}, v) + e$;
        \EndFor
        \State $v \gets $ \textbf{MinArg} $(M)$; \Comment{Find vertex that has minimum metric}
        \State \textbf{return } v 
       % \State \textbf{Return} v
   \end{algorithmic}
   \caption{ChooseVertex}\label{alg:ChooseVertex}
\end{algorithm}



\begin{algorithm}[H]
\begin{algorithmic}[1]
    \State \textbf{input } The root $v$, a set of leaves $\mathcal{L}$, the original graph $G=(V_G, E_G, \omega_G)$, and a Boolean $\Flip$.
    \State \textbf{output } The Steiner Tree  $T = (V_T, E_T, \omega_T)$, the path $\LeafPath$, and the set of Steiner nodes $\SteinerNodes$.
    \State $V_T, E_T \gets \{v:()\}, \{\}$;
    \State $\LeafPath,\SteinerNodes\gets(),()$; 
    \For{$u$ in $\mathcal{L}$}
    \State $\_, \paths \gets $\textbf{FindShortestPath}$(v, u, V_G, E_G)$;
    \For{$\pair$ in $\paths$}
    \State $V_T[\pair[0]] \gets V_T[\pair[0]].add(\pair[1])$;
    \If{$\pair[1]$ not in $V_T$}
    \State $V_T[\pair[1]]\gets()$;
    \EndIf
    \State $V_T[\pair[1]]\gets V_T[\pair[1]].add(\pair[0])$;
    \State $E_T[\pair]\gets E_G[\pair]$;
    \If{$\pair[1]$ not in $\mathcal{L}$ and not $v$}
    \State $\SteinerNodes \gets \SteinerNodes.add(\pair[1])$;
    \EndIf
    \If{$\Flip==\textbf{True}$}
    \State $\LeafPath \gets \LeafPath.add(\pair[1],\pair[0])$ \Comment{add flipped \pair}
    \Else
    \State $\LeafPath \gets \LeafPath.add(\pair)$
    \EndIf
    \EndFor
    % \State $\LeafPath \gets $\textbf{Union}$(\LeafPath, Paths)$;
    \EndFor 
    \State \textbf{return}  $(V_T, E_T, \LeafPath,\SteinerNodes)$
\end{algorithmic}
   \caption{ConstructSteinerTree}\label{alg:ConstructSteinerTree}
\end{algorithm}
%AccumulatedError
\begin{algorithm}[H]
   \begin{algorithmic}[1]
       \State \textbf{Input} Topology $G(V_G, E_G)$ with labels $l$, parity matrix $P$, vertex $v$
       \State \textbf{Output} Index $c$
       
        \State \textbf{Return} $c$
   \end{algorithmic}
   \caption{AccummulatedError}\label{alg:AccuulatedError}
    \end{algorithm}
    
\begin{algorithm}[H]
\begin{algorithmic}[1]
    \State \textbf{input } The connectivity graph $G=(V_G, E_G, \omega_G)$ with labels $q2v$, parity matrix \vect{A}, vertex $v$, and the index of the pivot column $c$.
    \State \textbf{output} The $\SteinerPath,$ and $\LeafPath$
    \State $r \gets $\textbf{IndexOf}$(q2v, v)$; 
    \State $\mathcal{L} \gets $ \textbf{FindLeavesinColumn}$(\vect{A}, r, c)$;
    \State $V_T, E_T, \LeafPath, \SteinerNodes \gets $\textbf{ConstructSteinerTree}$(v, \mathcal{L}, V_G, E_G, \Flip=$\textbf{False}$)$;
    \State $\SteinerPath \gets ()$;\Comment{Initialize $\SteinerPath$ with an empty set}    
    \State $\Candidates \gets \mathcal{L}.add(v)$;
    
    \For{ $u$ in $\SteinerNodes$} \Comment{Find paths to move parity of Steiner nodes to the leaves or root }
    \State $Weights, Paths, \MinPath \gets [],[],[]$;
    \For {$w$ in $\Candidates$} 
        
        \State $weight, Path \gets$\textbf{FindShortestPath}$ (w, u, V_T, E_T)$;
        \State $Weights \gets Weights + [weight]$;
        \State $Paths \gets Paths+[path]$;        
    \EndFor
    \State $\MinPath\gets Paths[$ \textbf{MinArg} $(Weights)]$
    \State $\SteinerPath \gets $ \textbf{union}$(\SteinerPath, \MinPath)$;
    \EndFor
    \State \textbf{return } $(\SteinerPath,\LeafPath)$
\end{algorithmic}
   \caption{Path2ReduceColumn}\label{alg:Path2ReduceColumn}
\end{algorithm}

 % ChooseColumn
\begin{algorithm}[H]
   \begin{algorithmic}[1]
       \State \textbf{Input} Topology $G(V_G, E_G)$ with labels $l$, parity matrix $P$, vertex $v$
       \State \textbf{Output} Index $c$ and $TotalPath$
       \State $r \gets l[v]$; \Comment{Find the row index corresponds to the vertex $v$}
       \State $\Candidates \gets \{\}$;
        \For {$i$ in $[0,...,|P[r]|]$}
            \If{$P[r, i]$ is $1$}
            \State $\Candidates[i]\gets 0$
            \EndIf
        \EndFor
        \For {$i$ in $\Candidates$}
            \State $\SteinerPath,\;\LeafPath\gets $\textbf{Path2ReduceColumn}$(v,i, P, G);$
            \State $TotalPath \gets \SteinerPath + \LeafPath;$
            \State $\Candidates[i] \gets $ (\textbf{AccumulatedError}$(TotalPath)$,$TotalPath)$; 
        \EndFor
        \State $c\gets $\textbf{MinArg}$(\Candidates);$
        \State \textbf{Return} $c,\;TotalPath$
   \end{algorithmic}
   \caption{ChooseColumn}\label{alg:ChooseColumn}
    \end{algorithm}
% \fi  

%ReduceColumn
\begin{algorithm}[H]
    \begin{algorithmic}[1]
        \State \textbf{Input} $\SteinerPath$, $\LeafPath$
       \State \textbf{Output} CNOT array $CNOTs_c$ 
       \State $CNOTs_c \gets []$; 
       \For {pair in reversed($\SteinerPath$)}
       \State $CNOTs_c \gets CNOTs_c  + [CNOT(pair[1], pair[0])]$
       \EndFor
       \For {pair in reversed($\LeafPath$)}
       \State $CNOTs_c \gets CNOTs_c  + [CNOT(pair[1], pair[0])]$
       \EndFor
%        \State $P, CNOTs_c = $ \textbf{addCNOT}$(pair, P, CNOTs_c)$;
%        \EndFor
    \end{algorithmic}
    \caption{ReduceColumn}\label{alg:ReduceColumn}
\end{algorithm}

  

\begin{algorithm}[H]
\begin{algorithmic}[1]
    \State \textbf{Input} Topology $G(V_G, E_G)$ with labels $q2v$, parity matrix $P$, vertex $v$, chosen column index $c$, output qubit map $m$
    \State \textbf{Output}$\SteinerPath,$ and $\LeafPath$
    \State $r \gets $\textbf{IndexOf}$(q2v, v)$; 
    \State $\mathcal{L} \gets $ \textbf{FindLeavesinRow}$(P, r, c, m)$;
    \State $V_T, E_T, \LeafPath, \SteinerNodes \gets $\textbf{ConstructSteinerTree}$(v, \mathcal{L}, V_G, E_G, \Flip=$\textbf{True}$)$;
    \State $\Candidates \gets \mathcal{L}.add(v)$;
    \For{ $u$ in $\SteinerNodes$} \Comment{Find paths to move parity of Steiner nodes to the leaves or root }
    \State $Weights, Paths, \MinPath \gets [],[],[]$;
    \For {$w$ in $\Candidates$} 
        
        \State $weight, Path \gets$\textbf{FindShortestPath}$ (u, w, V_T, E_T)$;
        \State $Weights \gets Weights + [weight]$;
        \State $Paths \gets Paths+[path]$;        
    \EndFor
    \State $\MinPath\gets Paths[$ \textbf{MinArg} $(Weights)]$
    \State $\SteinerPath \gets $ \textbf{union}$(\SteinerPath, \MinPath)$;
    \EndFor
   
    \State \textbf{Return} $\SteinerPath,$ and $\LeafPath$
\end{algorithmic}
   \caption{Path2ReduceRow}\label{alg:Path2ReduceRow}
\end{algorithm}

%ReduceOneQubit
\begin{algorithm}[H]
   \begin{algorithmic}[1]
       \State \textbf{Input} Topology $G(V_G, E_G)$, vertex $v$, chosen column index $c$, parity matrix $P$ with label $q2v$, paths to reduce column $\SteinerPath, \LeafPath$ 
       \State \textbf{Output} parity matrix $P$, CNOT array $CNOTs$ 
        % \State $P, CNOTs_c \gets $ \textbf{ReduceColumn}$(TotalPath)$ 
       \State$CNOTs_c \gets $ \textbf{ReduceColumn}( $\SteinerPath$, $\LeafPath$);
       \State $P \gets $\textbf{UpdateParity}$(P, q2v, CNOTs_c)$; \Comment{Apply row operations}
       \State $\SteinerPath, \LeafPath \gets $\textbf{Path2ReduceRow}$(V_G, E_G ,v, c, P, q2v, m);$
       \State$CNOTs_r \gets $ \textbf{ReduceRow}($\SteinerPath,\;\LeafPath$);
       \State $P \gets $\textbf{UpdateParity}$(P, q2v, CNOTs_r)$;\Comment{Apply row operations}
       \State $CNOTs \gets $\textbf{add}($CNOTs_c , CNOTs_r)$  \Comment{Concatenate CNOT lists}
        \State \textbf{Return} $P$, $CNOTs$
   \end{algorithmic}
   \caption{ReduceOneQubit}\label{alg:ReduceOneQubit}
    \end{algorithm}

    \begin{algorithm}[H]
\begin{algorithmic}[1]
    \State \textbf{Input} $\SteinerPath$, and $\LeafPath$
    \State\textbf{Output} CNOT array $CNOTs_r$

    \State $recover, CNOTs_r \gets [], []$;
    \For {pair in reversed($\SteinerPath$)} 
    \State $CNOTs_r \gets CNOTs_r  + [CNOT(pair[1], pair[0])]$
    % \State $P \gets $\textbf{RowOperation}$(P, v2q, pair)$;
        \If {pair[1] is not in $\mathcal{L}$ and not $v$}
        \State $recover \gets recover+[$pair$];$ \Comment{Recover parity of nodes that are not $\mathcal{L}$ and a root}
        \EndIf
    \EndFor
    \For {pair in reversed($recover$)}
    \State $CNOTs_r \gets CNOTs_r  + [CNOT(pair[1], pair[0])]$
    % \State $P \gets $\textbf{RowOperation}$(P, v2q, pair)$;
    \EndFor
    \For {pair in reversed($\LeafPath$)}
    \State $CNOTs_r \gets CNOTs_r  + [CNOT(pair[1], pair[0])]$
    % \State $P \gets $\textbf{RowOperation}$(P, v2q, pair)$;
    \EndFor
    \State \textbf{return} $CNOTs_r$
\end{algorithmic}
   \caption{ReduceRow}\label{alg:ReduceRow}
\end{algorithm}
%Main algorithm 
\begin{algorithm}[H]
   \begin{algorithmic}[1]
       \State \textbf{Input} Parity matrix $P$, topology $G(V_G, E_G)$ with labels $q2v$ corresponding to the rows of $P$
       \State \textbf{Output} CNOT array $CNOTs$ and output qubit map $m$
       % \State $C \gets$ new empty circuit; 
       \State $CNOTs,\; m\gets [ ],\;[-1,\; ...,\; -1]$;
       \While{$ |V_G|>1$}
       \State $v \gets $\textbf{ChooseVertex}$(G);$ 
       \State $c, \SteinerPath, \LeafPath \gets$\textbf{ChooseColumn}$(G,P,v,q2v);$
       \State $P, CNOTs' \gets$\textbf{ReduceOneQubit}$(v, c ,V_G, E_G, P, q2v, \SteinerPath, \LeafPath);$
       \State $CNOTs \gets$ \textbf{add}($CNOTs,\;CNOTs');$ \Comment{Extend list}
       \State $V_G, E_G \gets $\textbf{DeleteVertex}$(V_G, E_G, v);$
       \State $r \gets$ \textbf{IndexOf}($q2v,\;v$) \Comment{find index of $v$ in $q2v$}
       \State $m[c] \gets r;$
       \EndWhile
       \State $i \gets [i: i\in \{0, ...,   |m|-1\}$ where $m[i]=-1$]; 
       \State $m[i]\gets V_G[0];$ \Comment{Treat the final vertex}       
       \State \textbf{Return} $CNOTs, m$
   \end{algorithmic}
   \caption{Noise-Aware PermRowCol (NAPermRowCol)}\label{alg:NAPermRowCol}
    \end{algorithm}
    %\vspace{-1 em}
   % \scriptsize{Arianne \& Sarah: Dynamic qubit allocation and routing for constrained topologies by CNOT circuit re-synthesis. (2022)}



%Metric
\begin{algorithm}[H]
   \begin{algorithmic}[1]
       \State \textbf{Input} Topology $G(V_G, E_G)$ and the vertex $v$
       \State \textbf{Output} Average edge weight $m$ of the vertex
       \State $m \gets 0$;
       \State $degree \gets |v.neighbors|$;
            \For{$r$ in $v.neighbors$}
            \State $m\gets m + E_G[(v, r)]/degree$; \Comment{\small the average of edge weights.}
            \EndFor
        \State \textbf{Return} $m$
   \end{algorithmic}
   \caption{Metric}\label{alg:Metric}
    \end{algorithm}
% 
% 



% \iffalse







% \begin{algorithm}[H]
% \begin{algorithmic}[1]
%     \State \textbf{Input} vertex $v$, labels $q2v$, parity matrix $P$, output qubit map $m$
%     \State \textbf{Output} Set of leaves $leaves$ 
       % \Minyoung{Solve linear equations to solve} 
%     \State $row\_indices \gets [i: i \in (0, ..., n-1) $where $q2v[i]$ is not root and $m[i]$ is $-1$ (not located)$]$;
%     \State $column\_indices \gets [i: i \in (0, ..., n-1) $ where 
    
%     \State \textbf{Return}
% \end{algorithmic}
%    \caption{FindLeavesinRow}\label{alg:FindLeavesinRow}
% \end{algorithm}



%template
% \begin{algorithm}[H]
% \begin{algorithmic}[1]
%     \State \textbf{Input}
%     \State \textbf{Output}
%     \State \textbf{Return}
% \end{algorithmic}
%    \caption{title}\label{alg:title}
% \end{algorithm}


\iffalse
%Path2ReduceColumn
\begin{algorithm}[H]
   \begin{algorithmic}[1]
       \State \textbf{Input} Topology $G(V_G, E_G)$ with labels $q2v$, parity matrix $P$, vertex $v$
       \State \textbf{Output} cost $c$, $\SteinerPath,$ and $\LeafPath$
       \State $\mathcal{L} \gets $\textbf{Indexof1}$(P, $\textbf{IndexOf}$(l, v))$ \Comment{find leaves}
       \State $\SteinerNodes, \LeafPath \gets (), ()$ \Comment{Initialize $\SteinerNodes,\; \LeafPath$ with empty sets}
       \For{i in $\mathcal{L}$}
       \State $weight, Path \gets $\textbf{FindShortestPath}$(v, i, V_G, E_G)$;
       \For{edge in $Path$}
       \State $\LeafPath \gets \LeafPath.add($edge$)$;
       \If{edge[1] is not in $\mathcal{L}$ and not a root}
       \State $\SteinerNodes \gets \SteinerNodes.add($edge[1]$)$;
       \EndIf
       \EndFor
       \EndFor
       \State $\SteinerPath \gets ()$ \Comment{Initialize $\SteinerPath$ with an empty set}
       \State $\Candidates \gets \mathcal{L}.add(v)$;
    \For {$u$ in $SteinerNode$} \Comment{Find path to move parity of Steiner nodes to leaves or root }
        \State $Weights, Paths, \MinPath \gets [],[],[]$;
        \For {$w$ in $\Candidates$}
            \State $weight, Path \gets$
            \textbf{FindShortestPath}$ (u, w, V_G, E_G)$;
            \State $Weights \gets Weights + [weight]$;
            \State $Paths \gets Paths+[path]$;        
        \EndFor
        \State $\MinPath\gets Paths[$ \textbf{MinArg} $(Weights)]$
        \State $\SteinerPath \gets $ \textbf{union}$(\SteinerPath, \MinPath)$;
    \EndFor
        \State \textbf{Return} $c,\;\SteinerPath,\;\LeafPath$
   \end{algorithmic}
   \caption{Path2ReduceColumn}\label{alg:Path2ReduceColumn}
    \end{algorithm}
 %Path2ReduceRow
\begin{algorithm}[H]
   \begin{algorithmic}[1]
       \State \textbf{Input} 
       Topology $G(V_G, E_G)$, vertex $v$, chosen column index $c$, parity matrix $P$ with label $l$
       % Topology $G(V_G, E_G)$ with labels $l$, parity matrix $P$, vertex $v$
       \State \textbf{Output} $\mathcal{L}$, $\SteinerPath$, and $\LeafPath$
        \State $\mathcal{L} \gets $\textbf{FindLeavesinRow}$(P,l, v, c)$       
    % \State $A, B, NewLabel \gets $ \textbf{ReducedMatrix}$(P)$
    % \State $X \gets B \cdot$ \textbf{Inverse}$(A)$ \Comment{Solve linear equation to find leaves}
    % \State $\LeafPath,\;\SteinerNodes \gets (),()$ \Comment{Initialize $\LeafPath,\;\SteinerNodes$ with empty sets} 
    % \State $leaves \gets $\textbf{FindLeaf}$(l, X, NewLabel)$ \Comment{$leaves$ is a set of vertices where the component of $X$ is 1} 
    \For {$u$ in $\mathcal{L}$}
    \State $Path \gets $ \textbf{FindShortestPath}$(u, v, V_G, E_G)$
    \For {pair in $Path$}
        \State $\LeafPath \gets \LeafPath.add(pair)$ 
        \If {pair[1] is not in $\mathcal{L}$ and not $v$} 
        \State $SteinerNode \gets SteinerNode.add(pair[1])$ 
        \EndIf
    \EndFor
    \EndFor
    \State $\SteinerPath \gets ()$ \Comment{Initialize $\SteinerPath$ with an empty set }
    \State $\Candidates \gets \mathcal{L}.add(v)$;
    \For {$u$ in $SteinerNode$} \Comment{Find path to move parity of Steiner nodes to leaves or root }
        \State $Weights, Paths, \MinPath \gets [],[],[]$;
        \For {$w$ in $\Candidates$}
            \State $weight, Path \gets$
            \textbf{FindShortestPath}$ (u, w, V_G, E_G)$;
            \State $Weights \gets Weights + [weight]$;
            \State $Paths \gets Paths+[path]$;        
        \EndFor
        \State $\MinPath\gets Paths[$ \textbf{MinArg} $(Weights)]$
        \State $\SteinerPath \gets $ \textbf{union}$(\SteinerPath, \MinPath)$;
    \EndFor
       \State \textbf{Return} $\SteinerPath,\;\LeafPath\;,\mathcal{L}$
   \end{algorithmic}
   \caption{Path2ReduceRow}\label{alg:Path2ReduceRow}
    \end{algorithm}

%ReduceRow 
\begin{algorithm}[H]
\begin{algorithmic}[1]
    \State \textbf{Input}$\mathcal{L}$, $\SteinerPath$, and $\LeafPath$
    \State\textbf{Output} CNOT array $CNOTs_r$
    \State $recover, CNOTs_r \gets [], []$;
    \For {pair in $\SteinerPath$} 
    \State $CNOTs_r \gets CNOTs_r  + [CNOT(pair[1], pair[0])]$
        % \State $P, CNOTs_r = $ \textbf{addCNOT}$(pair, P, CNOTs_c)$;
        \If {pair[1] is not in $\mathcal{L}$ and not $v$}
        \State $recover \gets recover+[$pair$];$ \Comment{Recover parity of nodes that are not $\mathcal{L}$ and a root}
        \EndIf
    \EndFor
    \For {pair in $recover$}
    \State $CNOTs_r \gets CNOTs_r  + [CNOT(pair[1], pair[0])]$
    % \State $P, CNOTs_r = $ \textbf{addCNOT}$(pair, P, CNOTs_c)$;
    \EndFor
    \For {pair in $\LeafPath$}
    \State $CNOTs_r \gets CNOTs_r  + [CNOT(pair[1], pair[0])]$
    \EndFor
    % \State $P, CNOTs_r = $ \textbf{addCNOT}$(pair, P, CNOTs_c)$;
    \State \textbf{return} $CNOTs_r$
\end{algorithmic}
    \caption{ReduceRow}\label{alg:ReduceRow}
\end{algorithm}


\fi       

% 


==> scripts/8-2-comp.tex <==
\section{Complementary Benchmark Results}
\label{sec:complementarybenchmark}
Here we display the benchmark results on different backends. This means the topologies here are different from the one in \cref{sec:results}. The topology of each backend is displayed before the benchmark result. 
\subsection{Benchmark Results in Tables}
In this section, we display tables that record the benchmark results on the IBM FakeCairo, FakeMelbourne, and FakeNairobi backends. These tables demonstrate how we generate the benchmark circuits. They serve as the inputs to the algorithms \textit{NAPermRowCol}, \textit{PermRow}, and \textit{RowCol}.
\begin{table}[H]
    \centering
     \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5} & 2 & 8.0480 & 6.9615 & 6.5515\\
 & 4 & 11.7220 & 9.5755 & 9.0970\\
 & 5 & 13.0450 & 10.4250 & 9.9245\\
 & 8 & 16.3500 & 13.0010 & 12.1830\\
 & 10 & 17.2040 & 13.6430 & 12.6420\\
 & 15 & 18.1105 & 14.2035 & 12.7535\\
 & 20 & 19.2250 & 14.9410 & 13.8705\\
\hline
\multirow{5}{2em}{9} & 3 & 22.7725 & 21.0550 & 20.1245\\
 & 5 & 34.2680 & 30.0435 & 28.8045\\
 & 10 & 50.7475 & 44.7855 & 42.9950\\
 & 20 & 68.0080 & 59.1225 & 55.5835\\
 & 30 & 75.1640 & 66.3935 & 62.0345\\
\hline
\multirow{7}{2em}{16} & 4 & 58.0325 & 54.1290 & 51.9045\\
 & 8 & 101.7810 & 94.5690 & 87.9515\\
 & 16 & 161.8650 & 145.2665 & 134.6530\\
 & 32 & 220.0135 & 200.6835 & 188.8285\\
 & 64 & 266.2435 & 250.2595 & 235.3160\\
 & 128 & 282.2590 & 270.6010 & 253.7320\\
 & 256 & 284.1810 & 272.3585 & 256.4420\\
\hline
\multirow{7}{2em}{20} & 4 & 72.4650 & 68.6575 & 68.0615\\
 & 8 & 134.9105 & 126.8295 & 118.8305\\
 & 16 & 221.8790 & 205.3360 & 189.4025\\
 & 32 & 324.6530 & 297.5430 & 279.4000\\
 & 64 & 407.4445 & 384.5595 & 362.3370\\
 & 128 & 454.1085 & 439.7440 & 413.8330\\
 & 256 & 459.4055 & 447.5170 & 422.3395\\
        \hline
    \end{tabular}
    \caption{We compare our algorithm \textit{NAPermRowCol} against the algorithms \textit{PermRowCol}~\cite{griendli2022}, \textit{RowCol}~\cite{wu2023optimization}. The comparisons were made on IBM's FakeCairo backend, which hosts 27 qubits. The benchmarks were conducted on subregions of this topology involving 5, 9, 16, and 20 qubits, allowing for a comprehensive evaluation across varying circuit sizes and complexities. Consider a CNOT circuit over $m$ qubits, $m \in \{5,9,16,20\}$. For every $m$, we generate CNOT circuits whose original CNOT count is displayed in the second column. For each CNOT count, $100$ CNOT circuits are randomly generated. For each CNOT circuit, we generate $20$ initial maps with the numpy random module. Take benchmarking on a $5$-qubit subregion of the FakeCairo's topology as an example. We input $7\times100\times 20 = 14000$ CNOT circuits to the three algorithms listed in the table header. For example, when the original CNOT count is 2, there are $100\times 20 = 2000$ data points. We average them and obtain the benchmark results for each algorithm. On average, \textit{RowCol} produces 8.0480 CNOTs, \textit{PermRowCol} produces 6.9615 CNOTs, and \textit{NAPermRowCol} produces 6.5515 CNOT counts. The benchmark method is the same for different original CNOT counts.}
    \label{tab:CNOTCairo}
\end{table}
\subsection{Benchmark on the IBM's FakeMelbourne Backend}
\label{sec:melbourne}

We have benchmarked on IBM's FakeMelboure backend, as depicted in~\cref{fig:melbourne}. It hosts 15 qubits, and the details about the data generation are illustrated in~\cref{tab:CNOTMelbourne}.

\begin{figure}[H]
    \centering
   \includegraphics[scale=0.12]{graphics/melbourne.jpg} 
   %\includegraphics[width=1\textwidth]{graphics/melbourne.jpg}
% \vspace{.1 cm}
  \caption{The visualization of IBM's FakeMelbourne backend. It hosts 15 qubits, which correspond to 15 vertices in the connectivity graph. Since the quantum system is noisy, the error distribution is demonstrated by the different colouring of the edges. Here we only focus on the CNOT gate error rate, which corresponds to the colouring of the edges. The darker colour indicates the lower gate error rate.}
        \label{fig:melbourne}
\end{figure}
\begin{table}[H]
    \centering
     \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5}  & 2 & 7.5930 & 6.3975 & 6.1095\\
 & 4 & 11.1005 & 9.0445 & 8.7430\\
 & 5 & 12.4310 & 9.9840 & 9.5010\\
 & 8 & 15.6885 & 12.4020 & 11.6760\\
 & 10 & 16.4940 & 13.0370 & 12.1935\\
 & 15 & 17.2650 & 13.3025 & 12.3495\\
 & 20 & 18.6590 & 14.2935 & 13.1320\\
\hline
\multirow{5}{2em}{9} & 3 & 21.6875 & 19.8555 & 18.8650\\
 & 5 & 32.1010 & 28.0335 & 27.1535\\
 & 10 & 48.7720 & 41.9035 & 40.1625\\
 & 20 & 64.8295 & 55.9365 & 52.9450\\
 & 30 & 73.1985 & 63.8325 & 59.3470\\
\hline
        \hline
    \end{tabular}
    
    \caption{We compare our algorithm \textit{NAPermRowCol} against the algorithms \textit{PermRowCol}~\cite{griendli2022}, \textit{RowCol}~\cite{wu2023optimization}. The comparisons were made on IBM's FakeMelbourne backend, which hosts 15 qubits. The benchmarks were conducted on subregions of this topology involving 5, and 9 qubits, allowing for a comprehensive evaluation across varying circuit sizes and complexities. Consider a CNOT circuit over $m$ qubits, $m \in \{5,9,16,20\}$. For every $m$, we generate CNOT circuits whose original CNOT count is displayed in the second column. For each CNOT count, $100$ CNOT circuits are randomly generated. For each CNOT circuit, we generate $20$ initial maps with the numpy random module. Take benchmarking on a $5$-qubit subregion of the FakeCairo's topology as an example. We input $7\times100\times 20 = 14000$ CNOT circuits to the three algorithms listed in the table header. For example, when the original CNOT count is 2, there are $100\times 20 = 2000$ data points. We average them and obtain the benchmark results for each algorithm. On average, \textit{RowCol} produces 8.0480 CNOTs, \textit{PermRowCol} produces 6.9615 CNOTs, and \textit{NAPermRowCol} produces 6.5515 CNOT counts. The benchmark method is the same for different original CNOT counts.}
    \label{tab:CNOTMelbourne}
\end{table}
\begin{figure}[H]
% \renewcommand{\thefigure}{(a)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_melbourne_num_quibts=5_error probability.png}
% \vspace{.1 cm}
  \caption{The resynthesized circuits output from the four algorithms are compared in terms of the error probability as in \cref{lem:generalization}.}
        \label{fig:Melbourne5EP}
\end{subfigure}
% \renewcommand{\thefigure}{(b)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_melbourne_num_quibts=5_number of cnot.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the CNOT counts.}
        \label{fig:Melbourne5NC}
\end{subfigure}

\begin{subfigure}{1\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_melbourne_num_quibts=5_sum of cnot errors.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the accumulated CNOT gate error rates.}
        \label{fig:Melbourne5GER}
\end{subfigure}
% \renewcommand{\thefigure}{5}
\caption{The IBM's FakeMelbourne backend hosts $15$ qubits. Here, we benchmark on a $5$-qubit subregion of this topology, and compare our \textit{NAPermRowCol} against the state-of-the-art algorithms \textit{RowCol} and \textit{PermRowCol}, as well as the algorithm that lives in the Qiskit transpiler (short for `Qiskit').}
\end{figure}

\begin{figure}[H]
% \renewcommand{\thefigure}{(a)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_melbourne_num_quibts=9_error probability.png}
% \vspace{.1 cm}
  \caption{The resynthesized circuits output from the four algorithms are compared in terms of the error probability as in \cref{lem:generalization}.}
        \label{fig:Melbourne9EP}
\end{subfigure}
% \renewcommand{\thefigure}{(b)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_melbourne_num_quibts=9_number of cnot.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the CNOT counts.}
        \label{fig:Melbourne9NC}
\end{subfigure}

\begin{subfigure}{1\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_melbourne_num_quibts=9_sum of cnot errors.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the accumulated CNOT gate error rates.}
        \label{fig:Melbourne9GER}
\end{subfigure}
% \renewcommand{\thefigure}{5}
\caption{The IBM's FakeMelbourne backend hosts $15$ qubits. Here, we benchmark on a $9$-qubit subregion of this topology, and compare our \textit{NAPermRowCol} against the state-of-the-art algorithms \textit{RowCol} and \textit{PermRowCol}, as well as the algorithm that lives in the Qiskit transpiler (short for `Qiskit').}
\end{figure}


\iffalse
\begin{table}[H]
    \centering
     \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5}& 2 & 0.2291 & 0.1930 & 0.1869\\
 & 4 & 0.3359 & 0.2740 & 0.2657\\
 & 5 & 0.3778 & 0.3009 & 0.2880\\
 & 8 & 0.4767 & 0.3749 & 0.3563\\
 & 10 & 0.5021 & 0.3955 & 0.3712\\
 & 15 & 0.5253 & 0.4029 & 0.3767\\
 & 20 & 0.5682 & 0.4362 & 0.3988\\
\hline
\multirow{5}{2em}{9} & 3 & 0.6355 & 0.5805 & 0.5611\\
 & 5 & 0.9460 & 0.8233 & 0.8068\\
 & 10 & 1.4367 & 1.2304 & 1.1994\\
 & 20 & 1.9238 & 1.6558 & 1.5846\\
 & 30 & 2.1654 & 1.8855 & 1.7793\\
        \hline
    \end{tabular}
    \caption{sum of CNOT errors, Melbourne}
    \label{tab:SumCNOTMelbourne}
\end{table}
\begin{table}[H]
    \centering
   \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5} & 2 & 0.1994 & 0.1719 & 0.1678\\
 & 4 & 0.2794 & 0.2363 & 0.2310\\
 & 5 & 0.3084 & 0.2563 & 0.2479\\
 & 8 & 0.3754 & 0.3100 & 0.2990\\
 & 10 & 0.3922 & 0.3244 & 0.3096\\
 & 15 & 0.4064 & 0.3293 & 0.3137\\
 & 20 & 0.4326 & 0.3515 & 0.3290\\
\hline
\multirow{5}{2em}{9} & 3 & 0.4468 & 0.4186 & 0.4089\\
 & 5 & 0.5851 & 0.5372 & 0.5315\\
 & 10 & 0.7467 & 0.6910 & 0.6852\\
 & 20 & 0.8472 & 0.7998 & 0.7874\\
 & 30 & 0.8818 & 0.8425 & 0.8278\\
\hline
    \end{tabular}
    \caption{Error probability, Melbourne}
    \label{tab:errorprobabilityMelbourne}
\end{table}
\fi
\subsection{Benchmark on the IBM's FakeNairobi Backend}
\label{sec:nairobi}

\begin{figure}[H]
  \centering
  \includegraphics[scale=0.1]{graphics/nairobi.jpg}
  %[width=1\textwidth]{graphics/nairobi.jpg}
        \label{fig:nairobi}
\caption{The IBM's FakeNairobi backend hosts $7$ qubits. Here, we benchmark on a $5$-qubit subregion of this topology, and compare our \textit{NAPermRowCol} against the state-of-the-art algorithms \textit{RowCol} and \textit{PermRowCol}, as well as the algorithm that lives in the Qiskit transpiler (short for `Qiskit').}
\end{figure}

\begin{table}[H]
    \centering
     \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5} & 2 & 7.5930 & 6.3975 & 6.1095\\
 & 4 & 11.1005 & 9.0445 & 8.7430\\
 & 5 & 12.4310 & 9.9840 & 9.5010\\
 & 8 & 15.6885 & 12.4020 & 11.6760\\
 & 10 & 16.4940 & 13.0370 & 12.1935\\
 & 15 & 17.2650 & 13.3025 & 12.3495\\
 & 20 & 18.6590 & 14.2935 & 13.1320\\
\hline
    \end{tabular}
    \caption{CNOT counts, Nairobi}
    \label{tab:CNOTNairobi}
\end{table}

\begin{figure}[H]
% \renewcommand{\thefigure}{(a)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_nairobi_num_quibts=5_error probability.png}
% \vspace{.1 cm}
  \caption{The resynthesized circuits output from the four algorithms are compared in terms of the error probability as in \cref{lem:generalization}.}
        \label{fig:Nairobi5EP}
\end{subfigure}
% \renewcommand{\thefigure}{(b)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_nairobi_num_quibts=5_number of cnot.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the CNOT counts.}
        \label{fig:Nairobi5NC}
\end{subfigure}

\begin{subfigure}{1\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_nairobi_num_quibts=5_sum of cnot errors.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the accumulated CNOT gate error rates.}
        \label{fig:Nairobi5GER}
\end{subfigure}
% \renewcommand{\thefigure}{5}
\caption{The IBM's FakeNairobi backend hosts $7$ qubits. Here, we benchmark on a $5$-qubit subregion of this topology, and compare our \textit{NAPermRowCol} against the state-of-the-art algorithms \textit{RowCol} and \textit{PermRowCol}, as well as the algorithm that lives in the Qiskit transpiler (short for `Qiskit').}
\end{figure}

%\end{document}

\iffalse
\begin{table}[H]
    \centering
     \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5}& 2 & 0.0999 & 0.0869 & 0.0825\\
 & 4 & 0.1509 & 0.1188 & 0.1139\\
 & 5 & 0.1677 & 0.1319 & 0.1221\\
 & 8 & 0.2069 & 0.1645 & 0.1517\\
 & 10 & 0.2174 & 0.1734 & 0.1579\\
 & 15 & 0.2326 & 0.1780 & 0.1583\\
 & 20 & 0.2398 & 0.1881 & 0.1715\\
\hline
\multirow{5}{2em}{9} & 3 & 0.2771 & 0.2542 & 0.2336\\
 & 5 & 0.4172 & 0.3589 & 0.3369\\
 & 10 & 0.6151 & 0.5389 & 0.5073\\
 & 20 & 0.8286 & 0.7150 & 0.6594\\
 & 30 & 0.9093 & 0.8031 & 0.7343\\
\hline
\multirow{7}{2em}{16} & 4 & 0.7082 & 0.6625 & 0.5776\\
 & 8 & 1.2355 & 1.1468 & 0.9819\\
 & 16 & 1.9719 & 1.7635 & 1.4926\\
 & 32 & 2.6943 & 2.4461 & 2.0981\\
 & 64 & 3.2585 & 3.0692 & 2.6154\\
 & 128 & 3.4389 & 3.3135 & 2.8222\\
 & 256 & 3.4926 & 3.3479 & 2.8527\\
\hline
\multirow{7}{2em}{20} & 4 & 0.8909 & 0.8439 & 0.7598\\
 & 8 & 1.6558 & 1.5515 & 1.3294\\
 & 16 & 2.7253 & 2.5166 & 2.1197\\
 & 32 & 3.9865 & 3.6501 & 3.1057\\
 & 64 & 5.0331 & 4.7173 & 4.0284\\
 & 128 & 5.6357 & 5.4171 & 4.6266\\
 & 256 & 5.6716 & 5.5377 & 4.7202\\
        \hline
    \end{tabular}
    \caption{sum of CNOT errors, Cairo}
    \label{tab:SumCNOTCairo}
\end{table}

\begin{table}[H]
    \centering
   \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5} & 2 & 0.0931 & 0.0817 & 0.0783\\
 & 4 & 0.1374 & 0.1103 & 0.1065\\
 & 5 & 0.1513 & 0.1216 & 0.1137\\
 & 8 & 0.1838 & 0.1495 & 0.1395\\
 & 10 & 0.1921 & 0.1570 & 0.1448\\
 & 15 & 0.2044 & 0.1609 & 0.1452\\
 & 20 & 0.2100 & 0.1692 & 0.1564\\
\hline
\multirow{5}{2em}{9} & 3 & 0.2339 & 0.2175 & 0.2030\\
 & 5 & 0.3302 & 0.2925 & 0.2792\\
 & 10 & 0.4481 & 0.4074 & 0.3908\\
 & 20 & 0.5533 & 0.5016 & 0.4771\\
 & 30 & 0.5882 & 0.5429 & 0.5151\\
\hline
\multirow{7}{2em}{16} & 4 & 0.4849 & 0.4644 & 0.4234\\
 & 8 & 0.6889 & 0.6597 & 0.6096\\
 & 16 & 0.8457 & 0.8143 & 0.7637\\
 & 32 & 0.9257 & 0.9045 & 0.8710\\
 & 64 & 0.9576 & 0.9486 & 0.9233\\
 & 128 & 0.9645 & 0.9599 & 0.9379\\
 & 256 & 0.9665 & 0.9611 & 0.9400\\
\hline
\multirow{7}{2em}{20} & 4 & 0.5642 & 0.5439 & 0.5083\\
 & 8 & 0.7834 & 0.7612 & 0.7125\\
 & 16 & 0.9216 & 0.9046 & 0.8662\\
 & 32 & 0.9775 & 0.9686 & 0.9501\\
 & 64 & 0.9923 & 0.9893 & 0.9806\\
 & 128 & 0.9958 & 0.9947 & 0.9895\\
 & 256 & 0.9959 & 0.9953 & 0.9905\\
\hline
    \end{tabular}
    \caption{Error probability, Cairo}
    \label{tab:errorprobabilitycairo}
\end{table}
\fi


\iffalse
\begin{table}[H]
    \centering
     \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5}& 2 & 0.2291 & 0.1930 & 0.1869\\
 & 4 & 0.3359 & 0.2740 & 0.2657\\
 & 5 & 0.3778 & 0.3009 & 0.2880\\
 & 8 & 0.4767 & 0.3749 & 0.3563\\
 & 10 & 0.5021 & 0.3955 & 0.3712\\
 & 15 & 0.5253 & 0.4029 & 0.3767\\
 & 20 & 0.5682 & 0.4362 & 0.3988\\
        \hline
    \end{tabular}
    \caption{sum of CNOT errors, Nairobi}
    \label{tab:SumCNOTNairobi}
\end{table}
\begin{table}[H]
    \centering
   \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5}  & 2 & 0.1994 & 0.1719 & 0.1678\\
 & 4 & 0.2794 & 0.2363 & 0.2310\\
 & 5 & 0.3084 & 0.2563 & 0.2479\\
 & 8 & 0.3754 & 0.3100 & 0.2990\\
 & 10 & 0.3922 & 0.3244 & 0.3096\\
 & 15 & 0.4064 & 0.3293 & 0.3137\\
 & 20 & 0.4326 & 0.3515 & 0.3290\\
\hline
    \end{tabular}
    \caption{Error probability, Nairobi}
    \label{tab:errorprobabilityNairobi}
\end{table}
\fi




==> scripts/8-2-newcomp.tex <==
\section{Complementary Benchmark Results}
\label{sec:complementarybenchmark}
Here we display the benchmark results on different backends. This means the topologies here are different from the one in \cref{sec:results}. The topology of each backend is displayed before the benchmark result. 

\subsection{Benchmark on the IBM's Cairo Backend}
In this section, we display tables that record the benchmark results on the IBM FakeCairo. These tables demonstrate how we generate the benchmark figures. We compare our algorithm \textit{NAPermRowCol} against the algorithms \textit{PermRowCol}~\cite{griendli2022}, \textit{RowCol}~\cite{wu2023optimization}. The comparisons were made on IBM's FakeCairo backend, which hosts 27 qubits. The benchmarks were conducted on subregions of this topology involving 5, 9, 16, and 20 qubits, allowing for a comprehensive evaluation across varying circuit sizes and complexities. 
% They serve as the inputs to the algorithms \textit{NAPermRowCol}, \textit{PermRow}, and \textit{RowCol}.
\iffalse
\begin{figure}[H]
% \renewcommand{\thefigure}{(a)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.3]{graphics/fake_cairo_num_quibts=5_error probability.png}
% \vspace{.1 cm}
  \caption{The resynthesized circuits output from the four algorithms are compared in terms of the error probability as in \cref{def:generalization}.}
        \label{fig:Cairo5EP}
\end{subfigure}
% \renewcommand{\thefigure}{(b)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.3]{graphics/fake_cairo_num_quibts=5_number of cnot.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the CNOT counts.}
        \label{fig:Cairo5NC}
\end{subfigure}

\begin{subfigure}{1\textwidth}
  \centering
  \includegraphics[scale=0.3]{graphics/fake_cairo_num_quibts=5_sum of cnot errors.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the accumulated CNOT gate error rates.}
        \label{fig:Cairo5GER}
\end{subfigure}
% \renewcommand{\thefigure}{5}
\caption{The IBM's FakeCairo backend hosts $27$ qubits. Here, we benchmark on a $5$-qubit subregion of this topology, and compare our \textit{NAPermRowCol} against the state-of-the-art algorithms \textit{RowCol} and \textit{PermRowCol}, as well as the algorithm that lives in the Qiskit transpiler (short for `Qiskit').}

\label{fig:cairoquibts5}
\end{figure}


\begin{figure}[H]
% \renewcommand{\thefigure}{(a)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_cairo_num_quibts=9_error probability.png}
% \vspace{.1 cm}
  \caption{The resynthesized circuits output from the four algorithms are compared in terms of the error probability as in \cref{def:generalization}.}
        \label{fig:Cairo9EP}
\end{subfigure}
% \renewcommand{\thefigure}{(b)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_cairo_num_quibts=9_number of cnot.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the CNOT counts.}
        \label{fig:Cairo9NC}
\end{subfigure}

\begin{subfigure}{1\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_cairo_num_quibts=9_sum of cnot errors.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the accumulated CNOT gate error rates.}
        \label{fig:Cairo9GER}
\end{subfigure}
% \renewcommand{\thefigure}{5}
\caption{The IBM's FakeCairo backend hosts $27$ qubits. Here, we benchmark on a $9$-qubit subregion of this topology, and compare our \textit{NAPermRowCol} against the state-of-the-art algorithms \textit{RowCol} and \textit{PermRowCol}, as well as the algorithm that lives in the Qiskit transpiler (short for `Qiskit').}
\label{fig:cairoquibts9}
\end{figure}


\begin{figure}[H]
% \renewcommand{\thefigure}{(a)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_cairo_num_quibts=16_error probability.png}
% \vspace{.1 cm}
  \caption{The resynthesized circuits output from the four algorithms are compared in terms of the error probability as in \cref{def:generalization}.}
        \label{fig:Cairo16EP}
\end{subfigure}
% \renewcommand{\thefigure}{(b)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_cairo_num_quibts=16_number of cnot.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the CNOT counts.}
        \label{fig:Cairo16NC}
\end{subfigure}

\begin{subfigure}{1\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_cairo_num_quibts=16_sum of cnot errors.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the accumulated CNOT gate error rates.}
        \label{fig:Cairo16GER}
\end{subfigure}
% \renewcommand{\thefigure}{5}
\caption{The IBM's FakeCairo backend hosts $27$ qubits. Here, we benchmark on a $16$-qubit subregion of this topology, and compare our \textit{NAPermRowCol} against the state-of-the-art algorithms \textit{RowCol} and \textit{PermRowCol}, as well as the algorithm that lives in the Qiskit transpiler (short for `Qiskit').}
\label{fig:cairoquibts16}
\end{figure}

\begin{figure}[H]
% \renewcommand{\thefigure}{(a)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_cairo_num_quibts=20_error probability.png}
% \vspace{.1 cm}
  \caption{The resynthesized circuits output from the four algorithms are compared in terms of the error probability as in \cref{def:generalization}.}
        \label{fig:Cairo20EP}
\end{subfigure}
% \renewcommand{\thefigure}{(b)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_cairo_num_quibts=20_number of cnot.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the CNOT counts.}
        \label{fig:Cairo20NC}
\end{subfigure}

\begin{subfigure}{1\textwidth}
  \centering
  \includegraphics[scale=0.33]{graphics/fake_cairo_num_quibts=20_sum of cnot errors.png}
      \caption{The resynthesized circuits output from the four algorithms are compared in terms of the accumulated CNOT gate error rates.}
        \label{fig:Cairo20GER}
\end{subfigure}
% \renewcommand{\thefigure}{5}
\caption{The IBM's FakeCairo backend hosts $27$ qubits. Here, we benchmark on a $20$-qubit subregion of this topology, and compare our \textit{NAPermRowCol} against the state-of-the-art algorithms \textit{RowCol} and \textit{PermRowCol}, as well as the algorithm that lives in the Qiskit transpiler (short for `Qiskit').}

\label{fig:cairoquibts20}
\end{figure}
\fi

\begin{table}[H]
    \centering
     \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5} & 2 & 8.0480 & 6.9615 & 6.5515\\
 & 4 & 11.7220 & 9.5755 & 9.0970\\
 & 5 & 13.0450 & 10.4250 & 9.9245\\
 & 8 & 16.3500 & 13.0010 & 12.1830\\
 & 10 & 17.2040 & 13.6430 & 12.6420\\
 & 15 & 18.1105 & 14.2035 & 12.7535\\
 & 20 & 19.2250 & 14.9410 & 13.8705\\
\hline
\multirow{5}{2em}{9} & 3 & 22.7725 & 21.0550 & 20.1245\\
 & 5 & 34.2680 & 30.0435 & 28.8045\\
 & 10 & 50.7475 & 44.7855 & 42.9950\\
 & 20 & 68.0080 & 59.1225 & 55.5835\\
 & 30 & 75.1640 & 66.3935 & 62.0345\\
\hline
\multirow{7}{2em}{16} & 4 & 58.0325 & 54.1290 & 51.9045\\
 & 8 & 101.7810 & 94.5690 & 87.9515\\
 & 16 & 161.8650 & 145.2665 & 134.6530\\
 & 32 & 220.0135 & 200.6835 & 188.8285\\
 & 64 & 266.2435 & 250.2595 & 235.3160\\
 & 128 & 282.2590 & 270.6010 & 253.7320\\
 & 256 & 284.1810 & 272.3585 & 256.4420\\
\hline
\multirow{7}{2em}{20} & 4 & 72.4650 & 68.6575 & 68.0615\\
 & 8 & 134.9105 & 126.8295 & 118.8305\\
 & 16 & 221.8790 & 205.3360 & 189.4025\\
 & 32 & 324.6530 & 297.5430 & 279.4000\\
 & 64 & 407.4445 & 384.5595 & 362.3370\\
 & 128 & 454.1085 & 439.7440 & 413.8330\\
 & 256 & 459.4055 & 447.5170 & 422.3395\\
        \hline
    \end{tabular}
    \caption[Benchmark on the FakeCairo backend]{Consider a CNOT circuit over $m$ qubits, $m \in \{5,9,16,20\}$. For every $m$, we generate CNOT circuits whose original CNOT count is displayed in the second column. For each CNOT count, $100$ CNOT circuits are randomly generated. For each CNOT circuit, we generate $20$ initial maps with the numpy random module. Take benchmarking on a $5$-qubit subregion of the FakeCairo's topology as an example. We input $7\times100\times 20 = 14000$ CNOT circuits to the three algorithms listed in the table header. For example, when the original CNOT count is 2, there are $100\times 20 = 2000$ data points. We average them and obtain the benchmark results for each algorithm. On average, \textit{RowCol} produces 8.0480 CNOTs, \textit{PermRowCol} produces 6.9615 CNOTs, and \textit{NAPermRowCol} produces 6.5515 CNOT counts. The benchmark method is the same for different original CNOT counts.}
    \label{tab:CNOTCairo}
\end{table}
\subsection{Benchmark on the IBM's FakeMelbourne Backend}
\label{sec:melbourne}

We have benchmarked on IBM's FakeMelboure backend, as depicted in~\cref{fig:melbourne}. It hosts 15 qubits, and the details about the data generation are illustrated in~\cref{tab:CNOTMelbourne}.

\begin{figure}[H]
    \centering
   \includegraphics[scale=0.13]{graphics/melbourne.jpg} 
   %\includegraphics[width=1\textwidth]{graphics/melbourne.jpg}
% \vspace{.1 cm}
  \caption[The visualization of IBM's FakeMelbourne backend.]{The visualization of IBM's FakeMelbourne backend. It hosts 15 qubits, which correspond to 15 vertices in the connectivity graph. Since the quantum system is noisy, the error distribution is demonstrated by the different coloring of the edges. Here we only focus on the CNOT gate error rate, which corresponds to the coloring of the edges. The darker color indicates the lower gate error rate.}
        \label{fig:melbourne}
\end{figure}
\begin{table}[H]
    \centering
     \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5}  & 2 & 7.5930 & 6.3975 & 6.1095\\
 & 4 & 11.1005 & 9.0445 & 8.7430\\
 & 5 & 12.4310 & 9.9840 & 9.5010\\
 & 8 & 15.6885 & 12.4020 & 11.6760\\
 & 10 & 16.4940 & 13.0370 & 12.1935\\
 & 15 & 17.2650 & 13.3025 & 12.3495\\
 & 20 & 18.6590 & 14.2935 & 13.1320\\
\hline
\multirow{5}{2em}{9} & 3 & 21.6875 & 19.8555 & 18.8650\\
 & 5 & 32.1010 & 28.0335 & 27.1535\\
 & 10 & 48.7720 & 41.9035 & 40.1625\\
 & 20 & 64.8295 & 55.9365 & 52.9450\\
 & 30 & 73.1985 & 63.8325 & 59.3470\\
\hline
        \hline
    \end{tabular}
    
    \caption[Benchmark on the FakeMelbourne backend]{The benchmarks were conducted on subregions of this topology involving 5, and 9 qubits, allowing for a comprehensive evaluation across varying circuit sizes and complexities. Consider a CNOT circuit over $m$ qubits, $m \in \{5,9\}$. For every $m$, we generate CNOT circuits whose original CNOT count is displayed in the second column. For each CNOT count, $100$ CNOT circuits are randomly generated. For each CNOT circuit, we generate $20$ initial maps with the numpy random module. Take benchmarking on a $5$-qubit subregion of the FakeMelbourne's topology as an example. We input $7\times100\times 20 = 14000$ CNOT circuits to the three algorithms listed in the table header. For example, when the original CNOT count is 2, there are $100\times 20 = 2000$ data points. We average them and obtain the benchmark results for each algorithm. On average, \textit{RowCol} produces 7.5930 CNOTs, \textit{PermRowCol} produces 6.3975 CNOTs, and \textit{NAPermRowCol} produces 6.1095 CNOT counts. The benchmark method is the same for different original CNOT counts.}
    \label{tab:CNOTMelbourne}
\end{table}
\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.27]{graphics/fake_melbourne_num_quibts=5_error probability.png}
% \vspace{.1 cm}
  \subcaption{The resynthesized circuits output from the four algorithms are compared in terms of the error probability as in \cref{def:generalization}.}
        \label{fig:Melbourne5EP}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.27]{graphics/fake_melbourne_num_quibts=5_number of cnot.png}
      \subcaption{The resynthesized circuits output from the four algorithms are compared in terms of the CNOT counts.}
        \label{fig:Melbourne5NC}
\end{subfigure}

\begin{subfigure}{1\textwidth}
  \centering
  \includegraphics[scale=0.27]{graphics/fake_melbourne_num_quibts=5_sum of cnot errors.png}
      \subcaption{The resynthesized circuits output from the four algorithms are compared in terms of the accumulated CNOT gate error rates.}
        \label{fig:Melbourne5GER}
\end{subfigure}
\caption[Benchmark on a $5$-qubit subregion of FakeMelbourne backend]{The IBM's FakeMelbourne backend hosts $15$ qubits. Here, we benchmark on a $5$-qubit subregion of this topology, and compare our \textit{NAPermRowCol} against the state-of-the-art algorithms \textit{RowCol} and \textit{PermRowCol}, as well as the algorithm that lives in the Qiskit transpiler (short for `Qiskit').}
\end{figure}

\begin{figure}[H]
% \renewcommand{\thefigure}{(a)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.27]{graphics/fake_melbourne_num_quibts=9_error probability.png}
% \vspace{.1 cm}
  \subcaption{The resynthesized circuits output from the four algorithms are compared in terms of the error probability as in \cref{def:generalization}.}
        \label{fig:Melbourne9EP}
\end{subfigure}
% \renewcommand{\thefigure}{(b)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.27]{graphics/fake_melbourne_num_quibts=9_number of cnot.png}
      \subcaption{The resynthesized circuits output from the four algorithms are compared in terms of the CNOT counts.}
        \label{fig:Melbourne9NC}
\end{subfigure}

\begin{subfigure}{1\textwidth}
  \centering
  \includegraphics[scale=0.27]{graphics/fake_melbourne_num_quibts=9_sum of cnot errors.png}
      \subcaption{The resynthesized circuits output from the four algorithms are compared in terms of the accumulated CNOT gate error rates.}
        \label{fig:Melbourne9GER}
\end{subfigure}\
\caption[Benchmark on a $9$-qubit subregion of FakeMelbourne backend]{The IBM's FakeMelbourne backend hosts $15$ qubits. Here, we benchmark on a $9$-qubit subregion of this topology, and compare our \textit{NAPermRowCol} against the state-of-the-art algorithms \textit{RowCol} and \textit{PermRowCol}, as well as the algorithm that lives in the Qiskit transpiler (short for `Qiskit').}
\end{figure}


\iffalse
\begin{table}[H]
    \centering
     \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5}& 2 & 0.2291 & 0.1930 & 0.1869\\
 & 4 & 0.3359 & 0.2740 & 0.2657\\
 & 5 & 0.3778 & 0.3009 & 0.2880\\
 & 8 & 0.4767 & 0.3749 & 0.3563\\
 & 10 & 0.5021 & 0.3955 & 0.3712\\
 & 15 & 0.5253 & 0.4029 & 0.3767\\
 & 20 & 0.5682 & 0.4362 & 0.3988\\
\hline
\multirow{5}{2em}{9} & 3 & 0.6355 & 0.5805 & 0.5611\\
 & 5 & 0.9460 & 0.8233 & 0.8068\\
 & 10 & 1.4367 & 1.2304 & 1.1994\\
 & 20 & 1.9238 & 1.6558 & 1.5846\\
 & 30 & 2.1654 & 1.8855 & 1.7793\\
        \hline
    \end{tabular}
    \caption{sum of CNOT errors, Melbourne}
    \label{tab:SumCNOTMelbourne}
\end{table}
\begin{table}[H]
    \centering
   \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5} & 2 & 0.1994 & 0.1719 & 0.1678\\
 & 4 & 0.2794 & 0.2363 & 0.2310\\
 & 5 & 0.3084 & 0.2563 & 0.2479\\
 & 8 & 0.3754 & 0.3100 & 0.2990\\
 & 10 & 0.3922 & 0.3244 & 0.3096\\
 & 15 & 0.4064 & 0.3293 & 0.3137\\
 & 20 & 0.4326 & 0.3515 & 0.3290\\
\hline
\multirow{5}{2em}{9} & 3 & 0.4468 & 0.4186 & 0.4089\\
 & 5 & 0.5851 & 0.5372 & 0.5315\\
 & 10 & 0.7467 & 0.6910 & 0.6852\\
 & 20 & 0.8472 & 0.7998 & 0.7874\\
 & 30 & 0.8818 & 0.8425 & 0.8278\\
\hline
    \end{tabular}
    \caption{Error probability, Melbourne}
    \label{tab:errorprobabilityMelbourne}
\end{table}
\fi
\subsection{Benchmark on the IBM's FakeNairobi Backend}
\label{sec:nairobi}

\begin{figure}[H]
  \centering
  \includegraphics[scale=0.1]{graphics/nairobi.jpg}
  %[width=1\textwidth]{graphics/nairobi.jpg}
\caption[The visualization of IBM's FakeNairobi backend.]{The IBM's FakeNairobi backend hosts $7$ qubits. Here, we benchmark on a $5$-qubit subregion of this topology, and compare our \textit{NAPermRowCol} against the state-of-the-art algorithms \textit{RowCol} and \textit{PermRowCol}, as well as the algorithm that lives in the Qiskit transpiler (short for `Qiskit').}\label{fig:Nairobi5}
\end{figure}

\begin{table}[H]
    \centering
     \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5}  & 2 & 7.9795 & 6.8795 & 6.4360\\
 & 4 & 11.5965 & 9.5230 & 8.7630\\
 & 5 & 12.8985 & 10.4340 & 9.6990\\
 & 8 & 16.2060 & 12.9765 & 12.0070\\
 & 10 & 17.1650 & 13.7535 & 12.5960\\
 & 15 & 18.0095 & 13.8905 & 12.6810\\
 & 20 & 19.1210 & 14.8610 & 13.6695\\
\hline
    \end{tabular}
    \caption[Benchmark on the FakeNairobi backend]{The benchmarks were conducted on subregions of this topology involving 5 qubits, allowing for a comprehensive evaluation across varying circuit sizes and complexities. Consider a CNOT circuit over $5$ qubits, we generate CNOT circuits whose original CNOT count is displayed in the second column. For each CNOT count, $100$ CNOT circuits are randomly generated. For each CNOT circuit, we generate $20$ initial maps with the numpy random module. Take benchmarking on a $5$-qubit subregion of the FakeNairobi's topology as an example. We input $7\times100\times 20 = 14000$ CNOT circuits to the three algorithms listed in the table header. For example, when the original CNOT count is 2, there are $100\times 20 = 2000$ data points. We average them and obtain the benchmark results for each algorithm. On average, \textit{RowCol} produces 7.9795 CNOTs, \textit{PermRowCol} produces 6.8795 CNOTs, and \textit{NAPermRowCol} produces 6.4360 CNOT counts. The benchmark method is the same for different original CNOT counts.}
    \label{tab:CNOTNairobi}
\end{table}

%\end{document}

\iffalse
\begin{table}[H]
    \centering
     \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5}& 2 & 0.0999 & 0.0869 & 0.0825\\
 & 4 & 0.1509 & 0.1188 & 0.1139\\
 & 5 & 0.1677 & 0.1319 & 0.1221\\
 & 8 & 0.2069 & 0.1645 & 0.1517\\
 & 10 & 0.2174 & 0.1734 & 0.1579\\
 & 15 & 0.2326 & 0.1780 & 0.1583\\
 & 20 & 0.2398 & 0.1881 & 0.1715\\
\hline
\multirow{5}{2em}{9} & 3 & 0.2771 & 0.2542 & 0.2336\\
 & 5 & 0.4172 & 0.3589 & 0.3369\\
 & 10 & 0.6151 & 0.5389 & 0.5073\\
 & 20 & 0.8286 & 0.7150 & 0.6594\\
 & 30 & 0.9093 & 0.8031 & 0.7343\\
\hline
\multirow{7}{2em}{16} & 4 & 0.7082 & 0.6625 & 0.5776\\
 & 8 & 1.2355 & 1.1468 & 0.9819\\
 & 16 & 1.9719 & 1.7635 & 1.4926\\
 & 32 & 2.6943 & 2.4461 & 2.0981\\
 & 64 & 3.2585 & 3.0692 & 2.6154\\
 & 128 & 3.4389 & 3.3135 & 2.8222\\
 & 256 & 3.4926 & 3.3479 & 2.8527\\
\hline
\multirow{7}{2em}{20} & 4 & 0.8909 & 0.8439 & 0.7598\\
 & 8 & 1.6558 & 1.5515 & 1.3294\\
 & 16 & 2.7253 & 2.5166 & 2.1197\\
 & 32 & 3.9865 & 3.6501 & 3.1057\\
 & 64 & 5.0331 & 4.7173 & 4.0284\\
 & 128 & 5.6357 & 5.4171 & 4.6266\\
 & 256 & 5.6716 & 5.5377 & 4.7202\\
        \hline
    \end{tabular}
    \caption{sum of CNOT errors, Cairo}
    \label{tab:SumCNOTCairo}
\end{table}

\begin{table}[H]
    \centering
   \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5} & 2 & 0.0931 & 0.0817 & 0.0783\\
 & 4 & 0.1374 & 0.1103 & 0.1065\\
 & 5 & 0.1513 & 0.1216 & 0.1137\\
 & 8 & 0.1838 & 0.1495 & 0.1395\\
 & 10 & 0.1921 & 0.1570 & 0.1448\\
 & 15 & 0.2044 & 0.1609 & 0.1452\\
 & 20 & 0.2100 & 0.1692 & 0.1564\\
\hline
\multirow{5}{2em}{9} & 3 & 0.2339 & 0.2175 & 0.2030\\
 & 5 & 0.3302 & 0.2925 & 0.2792\\
 & 10 & 0.4481 & 0.4074 & 0.3908\\
 & 20 & 0.5533 & 0.5016 & 0.4771\\
 & 30 & 0.5882 & 0.5429 & 0.5151\\
\hline
\multirow{7}{2em}{16} & 4 & 0.4849 & 0.4644 & 0.4234\\
 & 8 & 0.6889 & 0.6597 & 0.6096\\
 & 16 & 0.8457 & 0.8143 & 0.7637\\
 & 32 & 0.9257 & 0.9045 & 0.8710\\
 & 64 & 0.9576 & 0.9486 & 0.9233\\
 & 128 & 0.9645 & 0.9599 & 0.9379\\
 & 256 & 0.9665 & 0.9611 & 0.9400\\
\hline
\multirow{7}{2em}{20} & 4 & 0.5642 & 0.5439 & 0.5083\\
 & 8 & 0.7834 & 0.7612 & 0.7125\\
 & 16 & 0.9216 & 0.9046 & 0.8662\\
 & 32 & 0.9775 & 0.9686 & 0.9501\\
 & 64 & 0.9923 & 0.9893 & 0.9806\\
 & 128 & 0.9958 & 0.9947 & 0.9895\\
 & 256 & 0.9959 & 0.9953 & 0.9905\\
\hline
    \end{tabular}
    \caption{Error probability, Cairo}
    \label{tab:errorprobabilitycairo}
\end{table}
\fi


\iffalse
\begin{table}[H]
    \centering
     \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5}& 2 & 0.2291 & 0.1930 & 0.1869\\
 & 4 & 0.3359 & 0.2740 & 0.2657\\
 & 5 & 0.3778 & 0.3009 & 0.2880\\
 & 8 & 0.4767 & 0.3749 & 0.3563\\
 & 10 & 0.5021 & 0.3955 & 0.3712\\
 & 15 & 0.5253 & 0.4029 & 0.3767\\
 & 20 & 0.5682 & 0.4362 & 0.3988\\
        \hline
    \end{tabular}
    \caption{sum of CNOT errors, Nairobi}
    \label{tab:SumCNOTNairobi}
\end{table}
\begin{table}[H]
    \centering
   \begin{tabular}{c|c|c|c|c}
        \hline
        number of qubits & CNOT counts  & RowCol & PermRowCol & NAPermRowCol \\
        \hline
        \multirow{7}{2em}{5}  & 2 & 0.1994 & 0.1719 & 0.1678\\
 & 4 & 0.2794 & 0.2363 & 0.2310\\
 & 5 & 0.3084 & 0.2563 & 0.2479\\
 & 8 & 0.3754 & 0.3100 & 0.2990\\
 & 10 & 0.3922 & 0.3244 & 0.3096\\
 & 15 & 0.4064 & 0.3293 & 0.3137\\
 & 20 & 0.4326 & 0.3515 & 0.3290\\
\hline
    \end{tabular}
    \caption{Error probability, Nairobi}
    \label{tab:errorprobabilityNairobi}
\end{table}
\fi

==> scripts/8-3-algowalkthrough.tex <==
\section{The NAPermRowCol Algorithm Walthrough}
\label{sec:algowalkthough}
In this section, we execute algorithm \textit{NAPermRowCol} with inputs, a CNOT circuit and the weighted topology graph of vertices ($G=(V_G, E_G, \omega_G)$). \cref{fig:walkthrough} describes the inputs to NAPermRowCol.





\begin{figure}[H]
  \begin{subfigure}[b]{1\textwidth}
  \centering
    \[
\Qcircuit @C=1.0em @R=1.02em @!R {
\lstick{\ket{q_0}}& \targ & \qw & \qw & \targ & \ctrl{3} & \qw & \qw & \qw & \qw & \qw &  \ctrl{1} & \qw & \targ & \qw &\rstick{\ket{q_0\oplus q_2\oplus q_4\oplus q_6}}\\
\lstick{\ket{q_1}}& \ctrl{-1} & \ctrl{2} & \ctrl{1} & \qw & \qw & \qw & \targ & \qw & \ctrl{1} & \ctrl{4} &  \targ & \qw & \qw & \qw &\rstick{\ket{q_0\oplus q_5\oplus q_6}}\\
\lstick{\ket{q_2}}& \qw & \qw & \targ & \qw & \qw & \ctrl{2} & \qw & \targ & \targ & \qw & \ctrl{4} &  \ctrl{3} & \qw & \qw &\rstick{\ket{q_0\oplus q_2\oplus q_3\oplus q_5\oplus q_6}}\\
\lstick{\vect{C}_0=\ket{q_3}}& \qw & \targ & \qw & \qw & \targ & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw &  \qw & \qw & \qw &\rstick{\ket{q_0\oplus q_3\oplus q_6}}\\
\lstick{\ket{q_4}}& \qw & \qw & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-4} & \qw &\rstick{\ket{q_1\oplus q_2\oplus q_4}}\\
\lstick{\ket{q_5}}& \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-4} & \qw & \qw & \targ & \qw &  \targ & \qw & \qw &\rstick{\ket{q_0\oplus q_1\oplus q_2\oplus q_3\oplus q_5\oplus q_6}}\\
\lstick{\ket{q_6}}& \qw & \qw & \qw & \ctrl{-6} & \qw & \qw & \qw & \qw & \qw & \qw & \targ & \qw &  \qw & \qw &\rstick{\ket{q_0\oplus q_2\oplus q_3\oplus q_5}}}
\]
\subcaption{The CNOT circuit $\vect{C}_0$ composed of $7$ qubits and $14$ $\CNOT$s. }\label{fig:7-qubit-cnot-circuit}
\end{subfigure}
  \begin{subfigure}[b]{0.5\textwidth}
 \centering
    \includegraphics[scale = .35]{graphics/initial_topology.png}
    \subcaption{The system snapshot of a fake 7-qubit IBM backend, Nairobi.}
    \label{fig:Nairobi}
  \end{subfigure}
  \begin{subfigure}[b]{0.5\textwidth}
  \[
\vect{A} = \begin{blockarray}{cccccccc}
& 0'& 1'& 2'& 3'& 4'& 5'& 6'\\
\begin{block}{c(ccccccc)}
0 & 1 & 1 & 1 & 1 & 0 & 1 & 1\\
1 & 0 & 0 & 0 & 0 & 1 & 1 & 0\\
2 & 1 & 0 & 1 & 0 & 1 & 1 & 1\\
3 & 0 & 0 & 1 & 1 & 0 & 1 & 1\\
4 & 1 & 0 & 0 & 0 & 1 & 0 & 0\\
5 & 0 & 1 & 1 & 0 & 0 & 1 & 1\\
6 & 1 & 1 & 1 & 1 & 0 & 1 & 0\\
\end{block}
\end{blockarray}
\]
\subcaption{Parity matrix $\vect{A}$}\label{fig:parityofC}
\end{subfigure}
\caption{(a) The input qubits are denoted on the left of the circuit. The output parity terms are denoted on the right of the circuit. (b) The snapshot of Nairobi contains important information about the quantum system such as the coupling map (i.e., the hardware topology) and the $\CNOT$ gate error rates. The blue indices label the vertices. Here, $V_G=\{\color{IMSBlue}0\color{black},\color{IMSBlue}1\color{black},\color{IMSBlue}2\color{black},\color{IMSBlue}3\color{black},\color{IMSBlue}4\color{black},\color{IMSBlue}5\color{black},\color{IMSBlue}6\color{black}\}$ and $E_G = \{(\color{IMSBlue}0\color{black},\color{IMSBlue}1\color{black}), (\color{IMSBlue}1\color{black},\color{IMSBlue}2\color{black}),(\color{IMSBlue}1\color{black},\color{IMSBlue}3\color{black}),(\color{IMSBlue}3\color{black},\color{IMSBlue}5\color{black}),(\color{IMSBlue}4\color{black},\color{IMSBlue}5\color{black}),(\color{IMSBlue}5\color{black},\color{IMSBlue}6\color{black})\}$ (c) Parity matrix \vect{A} of the circuit $\vect{C}_0$ depicted in (a)}
\label{fig:walkthrough}
\end{figure}

\subsection{The Initial Qubit Map for NAPermRowCol}
\label{subsec:initial mapping}
As an example, in \cref{tab: initial circuit placement}, logical qubit $i$ (coloured in green) is mapped to vertex $j$ (coloured in blue). 
\[
\Phi: \Z_7 \rightarrow \Z_7, \qquad \Phi(\color{IMSGreen}i\color{black})=\color{IMSBlue}j\color{black}.
\]
 %The blue colouring means that these indices are the labels of vertices and green colouring means that of logical qubits. 

\begin{table}[H]
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
Logical qubit $\color{IMSGreen}i$  & $\color{IMSGreen}0$ & $\color{IMSGreen}1$ & $\color{IMSGreen}2$ & $\color{IMSGreen}3$ & $\color{IMSGreen}4$ & $\color{IMSGreen}5$ & $\color{IMSGreen}6$ \\ \hline
Vertex $\color{IMSBlue}j$ & \color{IMSBlue}3 & \color{IMSBlue}4 & \color{IMSBlue}1 & \color{IMSBlue}2 & \color{IMSBlue}6 & \color{IMSBlue}5 & \color{IMSBlue}0 \\ \hline
\end{tabular}
\caption{The initial qubit map can be expressed as $\Phi=[\color{IMSBlue}3\color{black},\color{IMSBlue}4\color{black},\color{IMSBlue}1\color{black},\color{IMSBlue}2\color{black},\color{IMSBlue}6\color{black},\color{IMSBlue}5\color{black},\color{IMSBlue}0\color{black}]$.}
\label{tab: initial circuit placement}
\end{table}

Based on $\Phi$ and the hardware topology in \cref{fig:Nairobi with placement}, we show how to relabel the logical CNOT circuit and its parity matrix in \cref{fig:placements}.

\begin{figure}[H]
    \centering
     \includegraphics[scale =0.35]{graphics/topology.png}
    \caption{The IBM's FakeNairobi backend with logical qubits (in green) mapped to vertices (in blue). Each vertex corresponds to a quantum register. Each edge has a weight. It is the error rate $p$ when coupling the corresponding quantum registers. $p \in \R, 0 \leq p \leq 1$. $\{\color{IMSBlue}0,2,4,6\color{black}\}$ is the set of non-cutting vertices.}
    \label{fig:Nairobi with placement}
\end{figure}


\begin{figure}[!ht]    
\begin{subfigure}[b]{1\textwidth}
    \[
\Qcircuit @C=1em @R=1.02em @!R {
%0th
\lstick{\ket{q_{\color{IMSGreen}0\color{black}}}\xrightarrow{\Phi} \ket{q_{\color{IMSBlue}3\color{black}}}}& \targ & \qw & \qw & \targ & \ctrl{3} & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{1} & \qw & \targ & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}6\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
%1th
\lstick{\ket{q_{\color{IMSGreen}1\color{black}}}\xrightarrow{\Phi} \ket{q_{\color{IMSBlue}4\color{black}}}}  & \ctrl{-1} & \ctrl{2} & \ctrl{1} & \qw & \qw & \qw & \targ & \qw & \ctrl{1} & \ctrl{4} & \qw & \targ & \qw & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
%2nd
\lstick{\ket{q_{\color{IMSGreen}2\color{black}}}\xrightarrow{\Phi} \ket{q_{\color{IMSBlue}1\color{black}}}} & \qw & \qw & \targ & \qw & \qw & \ctrl{2} & \qw & \targ & \targ & \qw & \ctrl{4} & \qw & \ctrl{3} & \qw & \qw & \rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
%3th
\lstick{\vect{C}=\ket{q_{\color{IMSGreen}3\color{black}}}\xrightarrow{\Phi} \ket{q_{\color{IMSBlue}2\color{black}}}}& \qw & \targ & \qw & \qw & \targ & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw & \qw & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
%4th
\lstick{\ket{q_{\color{IMSGreen}4\color{black}}}\xrightarrow{\Phi} \ket{q_{\color{IMSBlue}6\color{black}}}} & \qw & \qw & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-4} & \qw  &\rstick{\ket{q_{\color{IMSBlue}4\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}6\color{black}}}}\\
%5th
\lstick{\ket{q_{\color{IMSGreen}5\color{black}}}\xrightarrow{\Phi} \ket{q_{\color{IMSBlue}5\color{black}}}}  & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-4} & \qw & \qw & \targ & \qw & \qw & \targ & \qw & \qw & \rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}4\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
%6th 
\lstick{\ket{q_{\color{IMSGreen}6\color{black}}}\xrightarrow{\Phi} \ket{q_{\color{IMSBlue}0\color{black}}}} & \qw & \qw & \qw & \ctrl{-6} & \qw & \qw & \qw & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}}}
        }
\]
\subcaption{$\vect{C}$ is the CNOT circuit to be routed by NAPermRowCol. On the lefthand side, after applying $\Phi$ to all logical qubits, the indices in $\vect{C}$ are updated. $\ket{q_{\color{IMSGreen}i\color{black}}}\xrightarrow{\Phi} \ket{q_{\color{IMSBlue}{j}}\color{black}}$ means that logical qubit \color{IMSGreen}i \color{black} is mapped to quantum register \color{IMSBlue}j\color{black}. On the righthand side, the output parity terms use the indices of the quantum registers.} 
\label{fig:7-qubit-relabelled-cnot-circuit}
\end{subfigure}

\vspace{.2 em}

 \begin{subfigure}[b]{1\textwidth}
  \[
% \vect{A} \xrightarrow[\text{Mapping}]{\text{Intial Qubit}}
\vect{A} = \begin{blockarray}{cccccccc}
& \color{IMSGreen}0'& \color{IMSGreen}1'& \color{IMSGreen}2'& \color{IMSGreen}3'& \color{IMSGreen}4'& \color{IMSGreen}5'& \color{IMSGreen}6'\\
\begin{block}{c(ccccccc)}
\color{IMSGreen}0 & 1 & 1 & 1 & 1 & 0 & 1 & 1\\
\color{IMSGreen}1 & 0 & 0 & 0 & 0 & 1 & 1 & 0\\
\color{IMSGreen}2 & 1 & 0 & 1 & 0 & 1 & 1 & 1\\
\color{IMSGreen}3 & 0 & 0 & 1 & 1 & 0 & 1 & 1\\
\color{IMSGreen}4 & 1 & 0 & 0 & 0 & 1 & 0 & 0\\
\color{IMSGreen}5 & 0 & 1 & 1 & 0 & 0 & 1 & 1\\
\color{IMSGreen}6 & 1 & 1 & 1 & 1 & 0 & 1 & 0\\
\end{block}
\end{blockarray}\qquad \xlongrightarrow{\Phi} \qquad \vect{A} = \begin{blockarray}{cccccccc}
&\color{IMSBlue} 3'& \color{IMSBlue}4'& \color{IMSBlue}1'& \color{IMSBlue}2'& \color{IMSBlue}6'& \color{IMSBlue}5'& \color{IMSBlue}0'\\
\begin{block}{c(ccccccc)}
\color{IMSBlue}3 & 1 & 1 & 1 & 1 & 0 & 1 & 1\\
\color{IMSBlue}4 & 0 & 0 & 0 & 0 & 1 & 1 & 0\\
\color{IMSBlue}1 & 1 & 0 & 1 & 0 & 1 & 1 & 1\\
\color{IMSBlue}2 & 0 & 0 & 1 & 1 & 0 & 1 & 1\\
\color{IMSBlue}6 & 1 & 0 & 0 & 0 & 1 & 0 & 0\\
\color{IMSBlue}5 & 0 & 1 & 1 & 0 & 0 & 1 & 1\\
\color{IMSBlue}0 & 1 & 1 & 1 & 1 & 0 & 1 & 0\\
\end{block}
\end{blockarray} 
 \]
% \vspace{-1.cm}
\subcaption{\vect{A} is the parity matrix representation of \vect{C}. Each column represents an output parity term and each row represents an input qubit state. On the lefthand side, the rows and columns of \vect{A} are indexed by the logical qubits (in green). After the initial qubit map $\Phi$, logical qubit \color{IMSGreen}$i$ \color{black} is mapped to quantum register \color{IMSBlue}$j$ \color{black}. On the righthand side, the rows and columns of \vect{A} are indexed by the physical qubits (in blue).}\label{fig:parity-qubit7}
\end{subfigure}
\caption{After an initial qubit map, logical qubits are mapped to the quantum registers in a NISQ hardware. Accordingly, the logical CNOT circuit \vect{C} has an updated parity matrix representation \vect{A} whose rows and columns are relabelled.} 
\label{fig:placements}
\end{figure}


\subsection{A Reduction Step}
\label{subsec:reduction step example}

\subsubsection{Select a Pivot Row and Column}
\label{subsubsec:pivot row and column selection}
Take \cref{fig:placements} for an example, consider choosing the pivots for the first reduction step. To choose a pivot row from $\vect{A}$, we start by considering the topology in \cref{fig:Nairobi with placement}. Its set of non-cutting vertices is $R_1 = \{\color{IMSBlue} 0,2,4,6\color{black}\}$. Correspondingly, we call them the \textit{non-cut rows} of \vect{A}. In \cref{fig: pivot row and pivot column selection}, the Hamming weights of these row are annotated in gray on the right of $\vect{A}$. Hence $R_2 = \{\color{IMSBlue}4\color{black}, \color{IMSBlue}6\color{black}\}$. Since both of them have degree 1, but vertex $\color{IMSBlue}4\color{black}$ has a smaller average incident edge weight (0.00619) than vertex $\color{IMSBlue}6\color{black}$ (0.00918), $R_3 = \{\color{IMSBlue}4\color{black}\}$. Therefore, row $\color{IMSBlue}4$ is the pivot row, $r = 4.$


To choose a pivot column from \vect{A}, consider the columns that have a $1$ in row $4$. Hence $C_1 = \{\color{IMSBlue}5'\color{black}, \color{IMSBlue}6'\color{black}\}$. For each column, build a Steiner tree and calculate the cost. Since column $\color{IMSBlue}5'$ induces the minimum cost, it is the pivot column and $c = 5$. \sarah{To be continued.}
\begin{figure}[H]
\[
\vect{A}=\begin{blockarray}{ccccccccc}
&\color{IMSBlue} 3'& \color{IMSBlue}4'& \color{IMSBlue}1'& \color{IMSBlue}2'& \color{IMSBlue}6'& \color{IMSRed}5'& \color{IMSBlue}0' & \color{IMSGray} \text{Candidate rows}\\
\begin{block}{c(ccccccc)c}
\color{IMSBlue}3 & 1 & 1 & 1 & 1 & 0 & \color{IMSRed}1 & 1 & \\
\color{IMSRed}4 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}1 & \color{IMSRed}1 & \color{IMSRed}0& \color{IMSGray}2\\
\color{IMSBlue}1 & 1 & 0 & 1 & 0 & 1 & \color{IMSRed}1 & 1& \\
\color{IMSBlue}2 & 0 & 0 & 1 & 1 & 0 & \color{IMSRed}1 & 1& \color{IMSGray}4\\
\color{IMSBlue}6 & 1 & 0 & 0 & 0 & 1 & \color{IMSRed}0 & 0& \color{IMSGray}2\\
\color{IMSBlue}5 & 0 & 1 & 1 & 0 & 0 & \color{IMSRed}1 & 1& \\
\color{IMSBlue}0 & 1 & 1 & 1 & 1 & 0 & \color{IMSRed}1 & 0& \color{IMSGray}5\\
\end{block}
\color{IMSGray}\text{Candidate columns} & & & & & \color{IMSGray}\checkmark & \color{IMSGray}\checkmark & \\
                %\color{IMSRed}\text{Column} & & & \color{IMSRed}\checkmark & &
\end{blockarray} \]
\caption{\vect{A} is the parity matrix before the first reduction step. On the right of \vect{A}, $\{2,4,2,5\}$ are the Hamming weights of the candidate rows. At the bottom of \vect{A}, a $\checkmark$ denotes a candidate column. The pivot row and column are selected and they are highlighted in red.}
\label{fig: pivot row and pivot column selection}
\end{figure}

\iffalse
\begin{description}
    \item[Select a pivot row and column.]\textbf{  }
\begin{description}
    \item[Step 1: ]Choose a pivot row from $\vect{A}$.
    \begin{description}
        \item[Step 1.1: ] From \cref{fig:Nairobi}, the set of non-cutting vertices is $\{\color{IMSBlue} 0,2,4,6\color{black}\}$. 
        \item[Step 1.2: ]The Hamming weights of each row that corresponds to the non-cutting vertex are expressed on the right side of the matrix $\vect{A}$, highlighted in orange. According to this, $R_2$ is the set of rows with labels $\color{IMSBlue}4\color{black}, \color{IMSBlue}6\color{black}$. 
        \item[Step 1.3: ] The both vertices have degree 1, but $\color{IMSBlue}4\color{black}$ has smaller average weight than $\color{IMSBlue}6\color{black}$. Hence the $R_3$ is the set of only one row with index $\color{IMSBlue}4$.
        \item[Step 1.3: ] Finally, the row with index $\color{IMSBlue}4$ is chosen as a pivot row.
    \end{description}
    \item[Step 2: ]Choose a pivot column from $\vect{A}$.
    \begin{description}
    \item[Step 2.1:]There are 2 non-zero values in the row with index $\color{IMSBlue}4$. Hence, $C_1$ is the set with columns with indices $\color{IMSBlue}5'\color{black}, \color{IMSBlue}6'\color{black}$. 
    \item[Step 2.2:] For each column, build a Steiner tree and calculate the cost. The details are described in \cref{alg:Path2ReduceColumn} and \cref{alg:ConstructSteinerTree}. 
    \item[Step 2.3:] According to the costs, the column with index $\color{IMSBlue}5'$ is chosen as a pivot column.
    \end{description}
\begin{figure}[H]
\[\begin{blockarray}{ccccccccc}
&\color{IMSBlue} 3'& \color{IMSBlue}4'& \color{IMSBlue}1'& \color{IMSBlue}2'& \color{IMSBlue}6'& \color{IMSRed}5'& \color{IMSBlue}0'\\
\begin{block}{c(ccccccc)c}
\color{IMSBlue}3 & 1 & 1 & 1 & 1 & 0 & \color{IMSRed}1 & 1 & \color{IMSOrange}/\\
\color{IMSRed}4 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}1 & \color{IMSRed}1 & \color{IMSRed}0& \color{IMSOrange}2\\
\color{IMSBlue}1 & 1 & 0 & 1 & 0 & 1 & \color{IMSRed}1 & 1& \color{IMSOrange}/\\
\color{IMSBlue}2 & 0 & 0 & 1 & 1 & 0 & \color{IMSRed}1 & 1& \color{IMSOrange}4\\
\color{IMSBlue}6 & 1 & 0 & 0 & 0 & 1 & \color{IMSRed}0 & 0& \color{IMSOrange}2\\
\color{IMSBlue}5 & 0 & 1 & 1 & 0 & 0 & \color{IMSRed}1 & 1& \color{IMSOrange}/\\
\color{IMSBlue}0 & 1 & 1 & 1 & 1 & 0 & \color{IMSRed}1 & 0& \color{IMSOrange}5\\
\end{block}
\end{blockarray} \]
\caption{Parity matrix $\vect{A}$ with a pivot row and a pivot column. The selected row and the column are highlighted in red. The numbers coloured orange on the right side of the matrix are Hamming weights of each row.}
\label{fig: pivot row and pivot column}
\end{figure}
\end{description}
\fi
\begin{description}
\item[Reduce the pivot column and the pivot row] \textbf{   }
% Consider the pivot column of index $c$ and the pivot row of index $r$. For brevity, denote them as $\mathbf{c}$ and $\mathbf{r}$ respectively.
\begin{description}
    \item[Step 1: ] Reduce the pivot column to a basis column vector whose r-indexed row has a $1$, and everywhere else has $0$'s. 
    \begin{figure}[H]
\begin{subfigure}[b]{1\textwidth}
    \centering
    \includegraphics[scale=.4]{graphics/topology_col_red.png}
    \caption{}
    
\end{subfigure}
\caption{Constructed Steiner tree for column reduction.}\label{fig:ST for column reduction}
% \label{fig:parity-col-red}
\end{figure}
    \begin{description}
        \item[Step 1.1: ] The index of the chosen column is $\color{IMSBlue}5'$. The rows with indices $\color{IMSBlue}0,1,2,3,5$ have 1 in the chosen column. The vertices with these labels are leaves. 
    \item[Step 1.2: ] The minimum Steiner tree with root $\color{IMSBlue}4$ and leaves, $\{\color{IMSBlue}0,1,2,3,5\color{black}\}$, is constructed and depicted in \cref{fig:ST for column reduction}.
    \item[Step 1.3: ] There is no Steiner node in this tree, thus, $\tau_1^s$ is an empty sequence, $\tau_1^s=\{\}$. \\And $\tau_1^l =\{(\color{IMSBlue}4, 5\color{black}), (\color{IMSBlue}5, 3\color{black}), (\color{IMSBlue}3, 1\color{black}), (\color{IMSBlue}1, 0\color{black}), (\color{IMSBlue}1, 2\color{black})\}$. The edges in $\tau_1^l$ are depicted in \cref{fig:ST for column reduction} as orange arrows.
    \item[Step 1.4: ]\cref{alg:ReduceColumn} reorders the edges in $\tau_1^s, \tau_1^l$ and gives a list of $\CNOT$s, \\$l_1 = [\CNOT(\color{IMSBlue}2, 1\color{black}), \CNOT(\color{IMSBlue}0, 1\color{black}), \CNOT(\color{IMSBlue}1, 3\color{black}), \CNOT(\color{IMSBlue}3, 5\color{black}), \CNOT(\color{IMSBlue}5, 4\color{black})]$.
    \item[Step 1.5: ]  Since each $\CNOT(u,v)$ corresponds to a row operation $R(v,u)$, \\the row operations $R(\color{IMSBlue}1, 2\color{black}), R(\color{IMSBlue}1, 0\color{black}), R(\color{IMSBlue}3, 1\color{black}), R(\color{IMSBlue}5, 3\color{black}), R(\color{IMSBlue}4, 5\color{black})$ are performed on $\vect{A}$ sequentially. This results in $\vect{A}_1$.
    \end{description}
    \item[Step 2: ] Reduce the pivot row to a basis row vector whose c-indexed column has a $1$, and everywhere else has $0$'s.
    \begin{figure}[H]
\begin{subfigure}[b]{1\textwidth}
    \centering
    \includegraphics[scale=.4]{graphics/topology_row_red.png}
\end{subfigure}
\caption{Constructed Steiner tree for row reduction.}
    \label{fig:ST for row reduction}
    % \caption{Reduce the pivot row. }
% \label{fig:parity-row-red}
\end{figure}
    \begin{description}
        \item[Step 2.1: ]The index of the chosen row is $\color{IMSBlue}4$. By solving the linear equation, we can find the leaves, $\color{IMSBlue}2, 3$. The vertices with these labels are leaves.
        \item[Step 2.2: ]The minimum Steiner tree with root $\color{IMSBlue}4$ and leaves, $\color{IMSBlue}2,3$ is constructed and depicted in \cref{fig:ST for row reduction}. There are two Steiner nodes $\color{IMSBlue}1,5$ coloured in gray.
        \item[Step 2.3: ]$\tau_2^s,\;\tau_2^l$ are found by \cref{alg:Path2ReduceRow}. $\tau_2^s=\{(\color{IMSBlue}5,4\color{black}),(\color{IMSBlue}1,2\color{black})\}$ is a sequence of edges which is the combined path from Steiner nodes to the leaves or the root. \\And $\tau_2^l =\{(\color{IMSBlue}2, 1\color{black}), (\color{IMSBlue}1, 3\color{black}), (\color{IMSBlue}3, 5\color{black}), (\color{IMSBlue}5, 4\color{black})\}$ is a sequence of edges which is the combined path from leaves to the root. The edges in both sequences ($\tau_2^s,\;\tau_2^l$) are depicted in \cref{fig:ST for row reduction} with yellow, orange arrows. 
        \item[Step 2.4: ]\cref{alg:ReduceRow} reorders the edges in $\tau_2^s, \tau_2^l$ and gives a list of $\CNOT$s, \\$l_2 = [\CNOT(\color{IMSBlue}4,5\color{black}),\CNOT(\color{IMSBlue}2,1\color{black}),\CNOT(\color{IMSBlue}1, 2\color{black}), \CNOT(\color{IMSBlue}3, 1\color{black}), \CNOT(\color{IMSBlue}5, 3\color{black}), \CNOT(\color{IMSBlue}4, 5\color{black})]$. 
        \item[Step 2.5: ] Since each $\CNOT(u,v)$ corresponds to a row operation $R(v,u)$, the row operations \\$R(\color{IMSBlue}5, 4\color{black}), R(\color{IMSBlue}1, 2\color{black}),R(\color{IMSBlue}2, 1\color{black}), R(\color{IMSBlue}1, 3\color{black}), R(\color{IMSBlue}3, 5\color{black}), R(\color{IMSBlue}5,4\color{black})$ are performed on $\vect{A}_1$ sequentially. This results in $\vect{A}_2$.
    \end{description}

\end{description}
    \begin{figure}[H]
    % \iffalse
    \begin{align}
    \vect{A} = \begin{blockarray}{cccccccc}
&\color{IMSBlue} 3'& \color{IMSBlue}4'& \color{IMSBlue}1'& \color{IMSBlue}2'& \color{IMSBlue}6'& \color{IMSRed}5'& \color{IMSBlue}0'\\
\begin{block}{c(ccccccc)}
\color{IMSBlue}3 & 1 & 1 & 1 & 1 & 0 & \color{IMSRed}1 & 1\\
\color{IMSRed}4 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}1 & \color{IMSRed}1 & \color{IMSRed}0\\
\color{IMSBlue}1 & 1 & 0 & 1 & 0 & 1 & \color{IMSRed}1 & 1\\
\color{IMSBlue}2 & 0 & 0 & 1 & 1 & 0 & \color{IMSRed}1 & 1\\
\color{IMSBlue}6 & 1 & 0 & 0 & 0 & 1 & \color{IMSRed}0 & 0\\
\color{IMSBlue}5 & 0 & 1 & 1 & 0 & 0 & \color{IMSRed}1 & 1\\
\color{IMSBlue}0 & 1 & 1 & 1 & 1 & 0 & \color{IMSRed}1 & 0\\
\end{block}
\end{blockarray}  & \xrightarrow[\;\;\;\;\substack{R(3, 1)\\ R(5, 3)\\ R(4, 5)}\;\;\;\;]{\substack{R(1, 2)\\ R(1, 0)}}\vect{A}_1 = \begin{blockarray}{cccccccc}
&\color{IMSBlue} 3'& \color{IMSBlue}4'& \color{IMSBlue}1'& \color{IMSBlue}2'& \color{IMSBlue}6'& \color{IMSRed}5'& \color{IMSBlue}0'\\
\begin{block}{c(ccccccc)}
\color{IMSBlue}3 & 1 & 0 & 0 & 1 & 0 & \color{IMSRed}0 & 0\\
\color{IMSRed}4 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}1 & \color{IMSRed}1 & \color{IMSRed}0\\
\color{IMSBlue}1 & 0 & 1 & 0 & 1 & 1 & \color{IMSRed}0 & 0\\
\color{IMSBlue}2 & 1 & 0 & 0 & 1 & 1 & \color{IMSRed}0 & 0\\
\color{IMSBlue}6 & 1 & 0 & 0 & 0 & 1 & \color{IMSRed}0 & 0\\
\color{IMSBlue}5 & 0 & 1 & 1 & 0 & 1 & \color{IMSRed}0 & 1\\
\color{IMSBlue}0 & 0 & 1 & 0 & 1 & 1 & \color{IMSRed}0 & 1\\
\end{block}
\end{blockarray} \nonumber\\ 
& \xrightarrow[\;\;\;\;\substack{R(2, 1)\\ R(1, 3)\\ R(3, 5)\\ R(5,4)}\;\;\;\;]{\substack{R(5, 4)\\ R(1, 2)}}\vect{A}_2 = \begin{blockarray}{cccccccc}
&\color{IMSBlue} 3'& \color{IMSBlue}4'& \color{IMSBlue}1'& \color{IMSBlue}2'& \color{IMSBlue}6'& \color{IMSRed}5'& \color{IMSBlue}0'\\
\begin{block}{c(ccccccc)}
\color{IMSBlue}3 & 0 & 0 & 0 & 0 & 1 & \color{IMSRed}0 & 0\\
\color{IMSRed}4 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}0 & \color{IMSRed}1 & \color{IMSRed}0\\
\color{IMSBlue}1 & 1 & 0 & 0 & 1 & 1 & \color{IMSRed}0 & 0\\
\color{IMSBlue}2 & 1 & 1 & 0 & 0 & 0 & \color{IMSRed}0 & 0\\
\color{IMSBlue}6 & 1 & 0 & 0 & 0 & 1 & \color{IMSRed}0 & 0\\
\color{IMSBlue}5 & 0 & 1 & 1 & 0 & 0 & \color{IMSRed}0 & 1\\
\color{IMSBlue}0 & 0 & 1 & 0 & 1 & 1 & \color{IMSRed}0 & 1\\
\end{block}
\end{blockarray} \nonumber
 \end{align}
 % \end{flushright}
 \caption{$\vect{A}$ is the parity matrix of the original circuit $\vect{C}_0$. The chosen column and row are highlighted in red. At step 1, a sequence of row operations is held, and it results in $\vect{A}_1$. Note that the chosen column with index $\color{IMSBlue}5'$ is a basis vector. Similarly, in step 2, a sequence of row operations is held and it results in $\vect{A}_2$.}
 \label{fig: parity matrix for row reduction}

\end{figure}
\item[Remove the reduced vertex from the topology]\textbf{   }
\begin{figure}[H]
    \centering
    \includegraphics[scale=.4]{graphics/topology_removed.png}
    \caption{Remove the reduced vertex from the topology. Vertex with index $\color{IMSBlue}4$ no longer participates in the subsequent reduction steps. It is removed from the topology. Now, the set of non-cutting vertices is $\{\color{IMSBlue} 0\color{black},\color{IMSBlue}2\color{black}, \color{IMSBlue}6\color{black}\}$}
    \label{fig:enter-label}
\end{figure}

\item[Concatenate the output CNOTs from the reduction step]\textbf{   }\\
From the previous step, we get two lists composed of \CNOT gates as follows. 
\begin{align}
l_1 &= [\CNOT(\color{IMSBlue}2, 1\color{black}), \CNOT(\color{IMSBlue}0, 1\color{black}), \CNOT(\color{IMSBlue}1, 3\color{black}), \CNOT(\color{IMSBlue}3, 5\color{black}), \CNOT(\color{IMSBlue}5, 4\color{black})]\nonumber\\
l_2 &= [\CNOT(\color{IMSBlue}4,5\color{black}),\CNOT(\color{IMSBlue}2,1\color{black}),\CNOT(\color{IMSBlue}1, 2\color{black}), \CNOT(\color{IMSBlue}3, 1\color{black}), \CNOT(\color{IMSBlue}5, 3\color{black}), \CNOT(\color{IMSBlue}4, 5\color{black})]\nonumber    
\end{align}
By sequentially concatenating the \CNOT in the list, we get the synthesized circuit depicted in \cref{fig:circuit after 1 reduction step}.
 % $ \CNOT(\color{IMSBlue}4, 5\color{black})\circ\CNOT(\color{IMSBlue}5, 3\color{black})\circ\CNOT(\color{IMSBlue}3, 1\color{black})\circ\CNOT(\color{IMSBlue}1, 2\color{black})\circ\CNOT(\color{IMSBlue}2,1\color{black})\circ\CNOT(\color{IMSBlue}4,5\color{black})\circ\CNOT(\color{IMSBlue}5, 4\color{black})\circ\CNOT(\color{IMSBlue}3, 5\color{black})\circ\CNOT(\color{IMSBlue}1, 3\color{black})\circ\CNOT(\color{IMSBlue}0, 1\color{black})\circ\CNOT(\color{IMSBlue}2, 1\color{black})$, 
\begin{figure}[H]
\[
\Qcircuit @C=1em @R=1.02em @!R {
\lstick{\ket{q_{\color{IMSBlue}3\color{black}}}}& \qw & \qw & \targ & \ctrl{5} & \qw \ar@{.}[]+<1em,1em>;[d]+<1em,-10em> & \qw & \qw & \qw & \ctrl{2} & \targ & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}4\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
\lstick{\ket{q_{\color{IMSBlue}4\color{black}}}}& \qw & \qw & \qw & \qw & \targ & \ctrl{4} & \qw & \qw & \qw & \qw & \ctrl{4} & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}4\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
\lstick{\ket{q_{\color{IMSBlue}1\color{black}}}}& \targ & \targ & \ctrl{-2} & \qw & \qw & \qw & \targ & \ctrl{1} & \targ & \qw & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}}}\\
\lstick{\vect{C} = \ket{q_{\color{IMSBlue}2\color{black}}}}& \ctrl{-1} & \qw & \qw & \qw & \qw & \qw & \ctrl{-1} & \targ & \qw & \qw & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
\lstick{\ket{q_{\color{IMSBlue}6\color{black}}}}& \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}6\color{black}}}}\\
\lstick{\ket{q_{\color{IMSBlue}5\color{black}}}}& \qw & \qw & \qw & \targ & \ctrl{-4} & \targ & \qw & \qw & \qw & \ctrl{-5} & \targ & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
\lstick{\ket{q_{\color{IMSBlue}0\color{black}}}}& \qw & \ctrl{-4} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}0\color{black}}}}}
\]

    \caption{Synthsized circuit. The left side of the dashed line is composed of \CNOT s from $l_1$ and the right side is composed of \CNOT s from $l_2$.}
    \label{fig:circuit after 1 reduction step}
\end{figure}
\end{description}
\subsection{After the reduction steps}
% \textbf{  \\}
After at most $n$ reduction steps, we have the synthesized circuit \vect{C} depicted in \cref{fig:final circuit} and the permutation matrix \vect{A} depicted in \cref{fig:permutation matrix}. 
\begin{figure}[H]
\begin{subfigure}[b]{1\textwidth}
\[
\scalebox{.78}{
\Qcircuit @C=0.5em @R=1.0em @!R {
\lstick{\ket{q_{\color{IMSBlue}3\color{black}}}}& \qw & \qw & \targ & \ctrl{5} & \qw & \qw & \qw & \qw & \ctrl{2} & \targ & \qw & \qw & \ctrl{5} & \targ & \ctrl{2} & \qw & \qw & \targ & \qw & \qw & \ctrl{5} & \targ & \qw & \qw & \ctrl{5} & \targ & \ctrl{2} & \qw & \targ & \qw & \ctrl{5} & \targ & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
\lstick{\ket{q_{\color{IMSBlue}4\color{black}}}}& \qw & \qw & \qw & \qw & \targ & \ctrl{4} & \qw & \qw & \qw & \qw & \ctrl{4} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}4\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
\lstick{\ket{q_{\color{IMSBlue}1\color{black}}}}& \targ & \targ & \ctrl{-2} & \qw & \qw & \qw & \targ & \ctrl{1} & \targ & \qw & \qw & \ctrl{1} & \qw & \qw & \targ & \targ & \ctrl{1} & \qw & \targ & \qw & \qw & \ctrl{-2} & \targ & \ctrl{4} & \qw & \qw & \targ & \ctrl{4} & \ctrl{-2} & \qw & \qw & \ctrl{-2} & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
\lstick{\vect{C} = \ket{q_{\color{IMSBlue}2\color{black}}}}& \ctrl{-1} & \qw & \qw & \qw & \qw & \qw & \ctrl{-1} & \targ & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \qw & \targ & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
\lstick{\ket{q_{\color{IMSBlue}6\color{black}}}}& \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \targ & \qw & \qw & \ctrl{1} & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}6\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}}\\
\lstick{\ket{q_{\color{IMSBlue}5\color{black}}}}& \qw & \qw & \qw & \targ & \ctrl{-4} & \targ & \qw & \qw & \qw & \ctrl{-5} & \targ & \qw & \targ & \ctrl{-5} & \qw & \qw & \qw & \ctrl{-5} & \qw & \ctrl{-1} & \targ & \qw & \qw & \qw & \targ & \ctrl{-5} & \qw & \qw & \qw & \ctrl{-1} & \targ & \qw & \targ & \qw &\rstick{\ket{q_{\color{IMSBlue}4\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}6\color{black}}}}\\
\lstick{\ket{q_{\color{IMSBlue}0\color{black}}}}& \qw & \ctrl{-4} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-4} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \qw & \qw & \qw &\rstick{\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}}}}}
\]
    \subcaption{The synthesized circuit after all reduction steps.}
    \label{fig:final circuit}
\end{subfigure}
\begin{subfigure}[b]{1\textwidth}
\[
\vect{A}=\begin{blockarray}{cccccccc}
& \color{IMSBlue}3'& \color{IMSBlue}4'& \color{IMSBlue}1'& \color{IMSBlue}2'& \color{IMSBlue}6'& \color{IMSBlue}5'& \color{IMSBlue}0'\\
\begin{block}{c(ccccccc)}
\color{IMSBlue}3 & 0 & 0 & 1 & 0 & 0 & 0 & 0\\
\color{IMSBlue}4 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\
\color{IMSBlue}1 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\
\color{IMSBlue}2 & 0 & 1 & 0 & 0 & 0 & 0 & 0\\
\color{IMSBlue}6 & 1 & 0 & 0 & 0 & 0 & 0 & 0\\
\color{IMSBlue}5 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\
\color{IMSBlue}0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\\
\end{block}
\end{blockarray}
\]
\subcaption{The permutation matrix results from reduction steps.}
\label{fig:permutation matrix}
\end{subfigure}
\caption{Outputs of the NAPermRowCol, the synthesized circuit \vect{C} and the permutation matrix \vect{A}. }
\end{figure}
\subsection{Relabelling of Logical qubits}
The permutation matrix gives information on how the logical qubits are relabelled. For example, the logical qubit with index $\color{IMSGreen}0\color{black}$ is mapped to the vertex with index $\color{IMSBlue}3\color{black}$ and $\color{IMSGreen}4\color{black}$ is mapped to the vertex with index $\color{IMSBlue}6\color{black}$. The first column in \vect{A} has 1 with row indexed $\color{IMSBlue}6\color{black}$. It means the evolved state of logical qubit with index $\color{IMSGreen}0\color{black}$, $\ket{q_{\color{IMSGreen}0\color{black}}\oplus q_{\color{IMSGreen}2\color{black}}\oplus q_{\color{IMSGreen}4\color{black}}\oplus q_{\color{IMSGreen}6\color{black}}}$ (with blue labels, $\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}6\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}$), is stored in the vertex $\color{IMSBlue}6\color{black}$. 
% \begin{figure}[H]
\begin{align}
\begin{blockarray}{cc}
\begin{block}{c|l}
\text{Initial state} & \text{Evolved state}\\\hline
    \ket{q_{\color{IMSGreen}0\color{black}}} & \ket{q_{\color{IMSGreen}0\color{black}}\oplus
q_{\color{IMSGreen}2\color{black}}\oplus q_{\color{IMSGreen}4\color{black}}\oplus q_{\color{IMSGreen}6\color{black}}}\\
    \ket{q_{\color{IMSGreen}1\color{black}}} & \ket{q_{\color{IMSGreen}0\color{black}}\oplus
q_{\color{IMSGreen}5\color{black}}\oplus q_{\color{IMSGreen}6\color{black}}}\\
    \ket{q_{\color{IMSGreen}2\color{black}}} & \ket{q_{\color{IMSGreen}0\color{black}}\oplus
q_{\color{IMSGreen}2\color{black}}\oplus q_{\color{IMSGreen}3\color{black}}\oplus q_{\color{IMSGreen}5\color{black}}\oplus q_{\color{IMSGreen}6\color{black}}}\\
    \ket{q_{\color{IMSGreen}3\color{black}}} & \ket{q_{\color{IMSGreen}0\color{black}}\oplus
q_{\color{IMSGreen}3\color{black}}\oplus q_{\color{IMSGreen}6\color{black}}}\\
    \ket{q_{\color{IMSGreen}4\color{black}}} & \ket{q_{\color{IMSGreen}1\color{black}}\oplus
q_{\color{IMSGreen}2\color{black}}\oplus q_{\color{IMSGreen}4\color{black}}}\\
    \ket{q_{\color{IMSGreen}5\color{black}}} & \ket{q_{\color{IMSGreen}0\color{black}}\oplus
q_{\color{IMSGreen}1\color{black}}\oplus q_{\color{IMSGreen}2\color{black}}\oplus q_{\color{IMSGreen}3\color{black}}\oplus q_{\color{IMSGreen}5\color{black}}\oplus q_{\color{IMSGreen}6\color{black}}}\\
    \ket{q_{\color{IMSGreen}6\color{black}}} & \ket{q_{\color{IMSGreen}0\color{black}}\oplus
q_{\color{IMSGreen}2\color{black}}\oplus q_{\color{IMSGreen}3\color{black}}\oplus q_{\color{IMSGreen}5\color{black}}}\\
\end{block}
\end{blockarray}
& \xrightarrow[\phi]{\text{Initial mapping}}
\begin{blockarray}{cc}
\begin{block}{c|l}
\text{Initial state} & \text{Evolved state}\\\hline
\ket{q_{\color{IMSBlue}3\color{black}}} & \ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}6\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}\\
\ket{q_{\color{IMSBlue}4\color{black}}} & \ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}} \\
\ket{q_{\color{IMSBlue}1\color{black}}} &
\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}\\
\ket{q_{\color{IMSBlue}2\color{black}}} & \ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}\\
 \ket{q_{\color{IMSBlue}6\color{black}}} & \ket{q_{\color{IMSBlue}4\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}6\color{black}}}\\
\ket{q_{\color{IMSBlue}5\color{black}}} & \ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}4\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}\\ 
\ket{q_{\color{IMSBlue}0\color{black}}} & \ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}}\\
\end{block}
\end{blockarray}\nonumber\\
 & \xrightarrow[]{\text{Permutation}}
\begin{blockarray}{l}
\begin{block}{l}
\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}\\
\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}4\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}\\
\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}\\
\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}\\
\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}6\color{black}}\oplus q_{\color{IMSBlue}0\color{black}}}\\
\ket{q_{\color{IMSBlue}4\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}6\color{black}}}\\
\ket{q_{\color{IMSBlue}3\color{black}}\oplus q_{\color{IMSBlue}1\color{black}}\oplus q_{\color{IMSBlue}2\color{black}}\oplus q_{\color{IMSBlue}5\color{black}}}\\ 
\end{block}
\end{blockarray}\nonumber
\end{align}
    % \caption{Caption}
    % \label{fig:enter-label}
% \end{figure}
\iffalse
After this reduction step, the logical value initially stored in the quantum register $r$ no longer participates in the subsequent logical operations. In other words, it will no longer be the supporting qubit of $\CNOT$s produced in the remaining reduction steps. Therefore, we say that vertex $r$ is reduced after this reduction step.

Since the quantum vertex with index $r$ no longer participates in the subsequent reduction steps, vertex $r$ should be removed from the $G = (V,E)$. Therefore, we update the topology for the next reduction step as $G = (V-\{r\},E-N(r))$, where $N(r)$ denotes all edges in $G$ that have $r$ as one of its end vertices.


\subsubsection{}
\label{sec:concatenatecnot}
After one reduction step, we obtain two lists of $\CNOT$ gates, where $l_1$ and $l_2$ resulted from the column and row reductions respectively. Suppose that $\lvert l_1\rvert = m_1$, $\lvert l_2\rvert = m_2$, and $l_{1_{[i]}}$ denotes the matrix form of row operation corresponding to the $\CNOT$ gate in $i$th index of the list $l_1$. Then, we have the following expressions:
% \vspace{-3.em}
\begin{align}
\bigotimes_{i=m_1-1}^{0}l_{1_{[i]}}\vect{A} =l_{1_{[m_1-1]}}...l_{1_{[0]}}\vect{A} = &  \mathbf{P_1},\quad \bigotimes_{j=m_2-1}^{0}l_{2_{[j]}}\mathbf{P_1} =l_{2_{[m_2-1]}}...l_{2_{[0]}} \mathbf{P_1} = \mathbf{P_2} \nonumber \\ 
     \text{and thus } & \bigotimes_{j=m_2-1}^{0}l_{2_{[j]}}\bigotimes_{i=m_1-1}^{0}l_{1_{[i]}}\vect{A} = \mathbf{P_2}
    \label{eqn:PtoP2}
\end{align}


According to \cref{subsec:synthesis}, we can find a list of $\CNOT$s by concatenating $l_1$ and $l_2$ sequentially. Let this new list be $l_3$. Then the $i$th component of $l_3$ is the $i$th component of $l_1$, and the $(m_1+j)$th component of $l_3$ is the $j$th component of $l_2$, $1 \leq i \leq m_1$ and $1 \leq j \leq m_2$.

Finally, \cref{eqn:PtoP2} is reduced to \cref{eqn:l3P}
% \vspace{-3.em}
\begin{equation}
\bigotimes_{i=(m_1+m_2-1)}^{0}l_{3_{[i]}}\mathbf{P}=\mathbf{P2}
    \label{eqn:l3P}
\end{equation}



\iffalse
\noindent\makebox[\textwidth]{\parbox{3\textwidth}{
\begin{align}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
$(u,v)\in E$  & $(0,1)$ & $(1,2)$ & $(1,3)$ & $(3,5)$ & $(4,5)$ & $(5,6)$ \\ \hline
$\omega(u,v)$ & 0.00777 & 0.00607 & 0.00792 & 0.01016 & 0.00619 & 0.00918 \\ \hline
\end{tabular}
\end{align}
}}\fi










\fi

==> scripts/8-6-summary-inputdata.tex <==
\section{Input Data for Simulation on IBM's Fake Backends}
\label{sec:input data}

\subsection{The Input Data for Comparing Different}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\begin{tabular}{|c|lll|}
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Circuit width n}} & \multicolumn{3}{c|}{The synthesized CNOT count}                                                         \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                               & \multicolumn{1}{c|}{Fake Nairobi (7 qubits)} & \multicolumn{1}{c|}{Fake Guadalupe (16 qubits)} & \multicolumn{1}{c|}{Fake Cairo (27 qubits)} \\ \hline
\multirow{19}{*}{$n =5$}& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{2  \quad (17)}& \multicolumn{1}{c|}{} \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{3  \quad (18)} & \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{4  \quad (48)} & \\ \cline{2-4} 
& \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{5  \quad (32)} & \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{6  \quad (21)} &  \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{7  \quad (21)} &  \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{8  \quad (30)} &  \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{9  \quad (51)} &  \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{10  \quad (47)} & \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{11  \quad (65)} & \\ \cline{2-4} 
& \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{12  \quad (50)} & \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{13  \quad (45)} &  \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{14  \quad (45)} &  \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{15  \quad (35)} &  \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{16  \quad (44)} &  \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{17  \quad (14)} &  \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{18  \quad (5)} &  \\ \cline{2-4} 
& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{19  \quad (7)} &  \\ \hline
\multirow{7}{*}{$n =6$}                              & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \cline{2-4} 
                                                     & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \cline{2-4} 
                                                     & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \cline{2-4} 
                                                     & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \cline{2-4} 
                                                     & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \cline{2-4} 
                                                     & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \cline{2-4} 
                                                     & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \hline
\multirow{6}{*}{$n =7$}                              & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \cline{2-4} 
                                                     & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \cline{2-4} 
                                                     & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \cline{2-4} 
                                                     & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \cline{2-4} 
                                                     & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \cline{2-4} 
                                                     & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}               &                                 \\ \hline
\end{tabular}
\end{table}

\subsection{The Input Data for Comparing Different Routing Algorithms}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\begin{tabular}{|l|lll|}
\hline
\multirow{2}{*}{Qubit width n} & \multicolumn{3}{c|}{The original CNOT count}                                                                            \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{Fake Nairobi (7 qubits)} & \multicolumn{1}{l|}{Fake Guadalupe (16 qubits)} & Fake Cairo (27 qubits) \\ \hline
\multirow{9}{*}{$n = 5$}       & \multicolumn{1}{l|}{4}                       & \multicolumn{1}{l|}{4}                          & 4                      \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{8}                       & \multicolumn{1}{l|}{8}                          & 8                      \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{16}                      & \multicolumn{1}{l|}{16}                         & 16                     \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{32}                      & \multicolumn{1}{l|}{32}                         & 32                     \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{64}                      & \multicolumn{1}{l|}{64}                         & 64                     \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{128}                     & \multicolumn{1}{l|}{128}                        & 128                    \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{256}                     & \multicolumn{1}{l|}{256}                        & 256                    \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{512}                     & \multicolumn{1}{l|}{512}                        & 512                    \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{1024}                    & \multicolumn{1}{l|}{1024}                       & 1024                   \\ \hline
\multirow{9}{*}{$n=7$}         & \multicolumn{1}{l|}{4}                       & \multicolumn{1}{l|}{4}                          & 4                      \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{8}                       & \multicolumn{1}{l|}{8}                          & 8                      \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{16}                      & \multicolumn{1}{l|}{16}                         & 16                     \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{32}                      & \multicolumn{1}{l|}{32}                         & 32                     \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{64}                      & \multicolumn{1}{l|}{64}                         & 64                     \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{128}                     & \multicolumn{1}{l|}{128}                        & 128                    \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{256}                     & \multicolumn{1}{l|}{256}                        & 256                    \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{512}                     & \multicolumn{1}{l|}{512}                        & 512                    \\ \cline{2-4} 
                               & \multicolumn{1}{l|}{1024}                    & \multicolumn{1}{l|}{1024}                       & 1024                   \\ \hline
\multirow{9}{*}{$n=16$}        & \multicolumn{1}{l|}{\multirow{9}{*}{}}       & \multicolumn{1}{l|}{4}                          & 4                      \\ \cline{3-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{8}                          & 8                      \\ \cline{3-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{16}                         & 16                     \\ \cline{3-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{32}                         & 32                     \\ \cline{3-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{64}                         & 64                     \\ \cline{3-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{128}                        & 128                    \\ \cline{3-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{256}                        & 256                    \\ \cline{3-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{512}                        & 512                    \\ \cline{3-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{1024}                       & 1024                   \\ \hline
\multirow{9}{*}{$n=20$}        & \multicolumn{1}{l|}{\multirow{9}{*}{}}       & \multicolumn{1}{l|}{\multirow{9}{*}{}}          & 4                      \\ \cline{4-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                           & 8                      \\ \cline{4-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                           & 16                     \\ \cline{4-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                           & 32                     \\ \cline{4-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                           & 64                     \\ \cline{4-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                           & 128                    \\ \cline{4-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                           & 256                    \\ \cline{4-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                           & 512                    \\ \cline{4-4} 
                               & \multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                           & 1024                   \\ \hline
\end{tabular}
\end{table}

==> scripts/Parallel.tex <==
\subsection{The Parallel Error Channels}
\label{subsec:parallel error channel}
A parallel error channel $\mathcal{E}_q$ is vertically composed of channels with arbitrary input and output dimensions. Let $d$ be its input dimension. As shown in \cref{fig:ParallelE}, $\mathcal{E}_0$ and $\mathcal{E}_1$ are two error channels followed by two ideal operations $\mathcal{U}_0$ and $\mathcal{U}_1$. $U_0$ and $U_1$ are their respective unitary matrix representations. Let $p_0$ and $p_1$ be the error rates of $\mathcal{E}_0$ and $\mathcal{E}_1$. Let $d_0$ and $d_1$ be the respectively input dimensions and $k \in \{0,1\}$. $d = d_0d_1$. By \cref{eqn:trace and epsilon}, we can express $\Tr[S_{\mathcal{E}_k}]$ in terms of $d_k$ and $p_k$.
\begin{align}
    \frac{\Tr[S_{\mathcal{E}_k}]}{d_k^2} = 1-\frac{d_k+1}{d_k}p_k. \label{eqn:trace and epsilon intermediate}
    %F_{ave}(\mathcal{E}_1, \mathcal{I}) & = 1-p_1 = \frac{\Tr[S_{\mathcal{E}_1}]}{d_1^2}\times \frac{d_1}{d_1+1} + \frac{1}{d_1+1}\nonumber\\
    %\rightarrow \; & \frac{\Tr[S_{\mathcal{E}_1}]}{d_1^2} = (1-p_1-\frac{1}{d_1+1})\times \frac{d_1+1}{d_1} = (1-\frac{d_1+1}{d_1}p_1) \label{eqn:trace and epsilon1}
\end{align}

\begin{figure}[H]
% \renewcommand{\thefigure}{(a)}
\begin{subfigure}{.5\textwidth}
  \centering
  \scalebox{1}{\tikzfig{graphics/circuits/parallel_channel}}
\vspace{.1 cm}
  \caption{The error channel $\mathcal{E}_q$ is vertically composed of two error channels $\mathcal{E}_0$ and $\mathcal{E}_1$, followed the respective ideal operations $\mathcal{U}_0$ and $\mathcal{U}_1$.}
  \label{fig:ParallelE}
\end{subfigure}%
% \renewcommand{\thefigure}{(b)}
\qquad
\begin{subfigure}{.5\textwidth}
  \centering
  \scalebox{1}{\tikzfig{graphics/circuits/parallel_channel_example}}
      \caption{$\mathcal{E}_q$ is composed of two noisy CNOTs. $p_0$ and $p_1$ are the error rates of $\mathcal{E}_0^{\text{CNOT}}$ and $\mathcal{E}_1^{\text{CNOT}}$.}
    \label{fig:ParallelECNOT}
\end{subfigure}
% \renewcommand{\thefigure}{5}
\caption{The parallel error channels.}
\end{figure}

%Consider error channels $\mathcal{E}_0$ and $\mathcal{E}_1$ alongside Clifford gates $U_0$ and $U_1$  without errors, as shown in \cref{fig:ParallelE}. 
%Then, assign gate error rates $p_0$ and $p_1$, and input dimensions $d_0$ and $d_1$ to the respective error channels. 

In \cref{fig:ParallelECNOT}, consider an example when $\mathcal{E}_q$ is vertically composed of two noisy CNOT channels. Then 
\[
\mathcal{E}_q =\mathcal{E}_0 \otimes \mathcal{E}_1,\;\; d = d_0d_1,\;\; d_0 = d_1 = 4, \;\; \text{ and } \;\; U_0 = U_1 = \text{CNOT}.
\]

   

\begin{lemma}
    \lempara
    \label{lem:average fidelity parallel}
\end{lemma}


\begin{proof}
    Using \cref{eqn:trace and epsilon,eqn:trace and epsilon intermediate}, we can calculate the average gate fidelity of $\mathcal{E}_q$ over all possible input states. Moreover, we use the property that $\Tr[A\otimes B] = \Tr[A]\Tr[B]$ for matrices $A$ and $B$. More details can be found in \cref{sec: proof of claim}.


%if we take the CNOT error channel as the upper channel, $\mathcal{E}_0$ is the error channel, $d_0$ is $4$, and the Clifford gate $U_0$ is the CNOT gate. The composite error channel $\mathcal{E}_q$ results from the tensor product of the two error channels, $\mathcal{E}_0$ and $\mathcal{E}_1$. Leveraging the property $\Tr[A\otimes B] = \Tr[A]\Tr[B]$ for matrices $A$ and $B$, the average gate fidelity of $\mathcal{E}_q$ results in \cref{eqn: approximated form of parallel channels} utilizing \cref{eqn:trace and epsilon} where $k \in \{0,1\}$.

% simple version 
\begin{align}
    F_{ave}(\mathcal{E}_q) & =F_{ave}(\mathcal{E}_0 \otimes \mathcal{E}_1) = \frac{\Tr[S_{\mathcal{E}_0}\otimes S_{\mathcal{E}_1}]}{(d_0d_1)^2}\times \frac{d_0d_1}{d_0d_1+1} + \frac{1}{d_0d_1+1}\nonumber\\
    & =\frac{ \Tr[S_{\mathcal{E}_0}] \Tr[S_{\mathcal{E}_1}]}{(d_0d_1)^2}\times \frac{d_0d_1}{d_0d_1+1} + \frac{1}{d_0d_1+1}\nonumber\\
    & = 1-p_0 -p_1 + p_0p_1 + \frac{(1-d_1)p_0 + (1-d_0)p_1 + (d_0+d_1)p_0p_1}{d_0d_1+1}\nonumber\\
    %& = 1-(p_0+p_1) + O\bigl(\max\{p_0p_1,p_0/d_0,p_1/d_1\}\bigr).
    &= 1 - (p_0 + p_1) + \max\Biggl\{O\biggl(\frac{p_0}{d_0}\biggr), O\biggl(\frac{p_1}{d_1}\biggr), O(p_0p_1)\Biggr\}.
     \label{eqn: approximated form of parallel channels}
\end{align}
\end{proof}
% % %detail version 

Let $\Prob(\mathcal{E}_q)$ be the error probability of the parallel error channel $\mathcal{E}_q$. According to \cref{eqn: approximated form of parallel channels}, we have derived the approximated expression for its average gate fidelity. By \cref{eqn: gate error},



\begin{equation}
    \Prob(\mathcal{E}_q)=(p_0 + p_1) - \max\Biggl\{O\biggl(\frac{p_0}{d_0}\biggr), O\biggl(\frac{p_1}{d_1}\biggr), O(p_0p_1)\Biggr\}.
    \label{eq:error original} 
\end{equation}

Depending on the specific values of $p_0, p_1, d_0$ and $d_1$, the approximated form of \cref{eqn: approximated form of parallel channels} could be simplified as $(1-p_0)(1-p_1)$ or $1-(p_0+p_1)$. When $O(p_0p_1)$ takes the dominance, we derive \cref{eq:error} and refer to $(1-p_0)(1-p_1)$ as the success rate. Otherwise, we derive \cref{eq:error alt} and refer to $1 - (p_0 + p_1)$ as the success rate.
\begin{align}
    \Prob(\mathcal{E}_q) \approx (p_0 + p_1) - p_0p_1 = 1 - (1-p_0)(1-p_1)\label{eq:error} 
\end{align}


\begin{align}
    \Prob(\mathcal{E}_q) \approx p_0 + p_1.
    \label{eq:error alt} 
\end{align}

Note that choosing which simplified form depends on the magnitude of the individual gate error rate and the number of qubits in the circuit. In \cref{sec:results}, we benchmark with CNOT gates whose error probability is around $10^{-1}$. Since $d_0, d_1 \geq \log(10) \approx 3$, \cref{eq:error} holds for a CNOT circuit over more than $3\times2 = 6$ qubits. Therefore, we chose circuits of size $7$, $15$, and $27$ and use \cref{eq:error} for our cost function.


==> scripts/alternative_proof.tex <==
\iffalse
\sarah{There are two ways to derive the bounds. Both are correct, but we will have a slightly different argument. Below is the first version.}


\begin{proposition}
Let $\Prob(\mathcal{E}_c)$ be the error probability of the consecutive error channel $\mathcal{E}_c$. Then
\[
F_{ave}(\mathcal{E}_c) =  1-(p_0+p_1) + O(p_0p_1),\qquad \Prob(\mathcal{E}_c)\approx p_0 + p_1.
\]
\label{pro:approximate fidelity Ec}
\end{proposition}

\begin{proof}
%simple version 

By \cref{eqn: trace,eqn:trace and epsilon}, we have
    \begin{align}
    F_{ave}(\mathcal{E}_c, \mathcal{I}) & =(\Tr[S_{\mathcal{E}_0}]+\Tr[S_{\mathcal{E}_1}]-d^2+\Tr[A_1A_0] )\times \frac{1}{d(d+1)} + \frac{1}{d+1}\nonumber\\
     &  = \Biggl(d^2 \Bigl(1-\frac{d+1}{d}p_0\Bigr)+d^2 \Bigl(1-\frac{d+1}{d}p_1\Bigr)-d^2\Biggr)\frac{1}{d(d+1)}  +  \frac{Tr[A_1A_0]}{d(d+1)}+ \frac{1}{d+1}\nonumber\\
      & =  1-p_0-p_1 +  \frac{Tr[A_1A_0]}{d(d+1)}.\nonumber\\
    % &  = (d^2 (1-\frac{d+1}{d}p_0)+d^2 (1-\frac{d+1}{d}p_1)-d^2)\times\frac{1}{d(d+1)}  +  \Tr[A_1A_0]\frac{1}{d(d+1)}+ \frac{1}{d+1}\nonumber\\
 % & =  1-p_0-p_1 +  \frac{1}{d(d+1)}\Tr[A_1A_0]\nonumber\\
 \label{eqn: helper}
 \end{align}
 Combining \cref{lem:bound,eqn: helper}, we get
 \begin{align}
 1-p_0-p_1+p_0p_1+ \frac{1}{d}p_0p_1 \leq F_{ave}(\mathcal{E}_c, \mathcal{I}) \leq 1-p_0-p_1+2p_0p_1+\frac{2}{d}p_0p_1.\label{eqn: mid}
\end{align}
 Since $d \geq 1$ and $0<p_0, p_1 <1$, \cref{eqn: mid} can be further bounded as
 \[
 -4p_0p_1\leq p_0p_1+\frac{1}{d}p_0p_1\leq \bigl[F_{ave}(\mathcal{E}_c, \mathcal{I})-(1-p_0-p_1)\bigr] \leq 2p_0p_1 + \frac{2}{d}p_0p_1 \leq 4p_0p_1.
 \]
 It follows that 
 \[
  F_{ave}(\mathcal{E}_c, \mathcal{I})-(1-p_0-p_1) = O(p_0p_1).
 \]
Therefore, $F_{ave}(\mathcal{E}_c, \mathcal{I}) =  1-(p_0+p_1) + O(p_0p_1)$.

According to \cref{pro:approximate fidelity Ec}, since $p_0p_1 < p_0$ and $p_0p_1 < p_1$, we derive the same approximated expression for the average gate fidelity as did in \cref{eq:error alt}.
\begin{equation}
    \Prob(\mathcal{E}_c)\approx p_0 + p_1.
    \label{eq:consecutive error rate} 
\end{equation}

\end{proof}









\sarah{Below is the previous version: $F_{ave}(\mathcal{E}_c, \mathcal{I}) =  1-(p_0+p_1) +  p_0p_1 + O(p_0p_1)$. This provides a tighter bound than the above version.}
\fi

